Improved Distributed Expander Decomposition and Nearly Optimal Triangle Enumeration

An $(\epsilon,\phi)$-expander decomposition of a graph $G=(V,E)$ is a clustering of the vertices $V=V_{1}\cup\cdots\cup V_{x}$ such that (1) each cluster $V_{i}$ induces subgraph with conductance at least $\phi$, and (2) the number of inter-cluster edges is at most $\epsilon|E|$. In this paper, we give an improved distributed expander decomposition. Specifically, we construct an $(\epsilon,\phi)$-expander decomposition with $\phi=(\epsilon/\log n)^{2^{O(k)}}$ in $O(n^{2/k}\cdot\text{poly}(1/\phi,\log n))$ rounds for any $\epsilon\in(0,1)$ and positive integer $k$. For example, a $(0.01,1/\text{poly}\log n)$-expander decomposition can be computed in $O(n^{\gamma})$ rounds, for any arbitrarily small constant $\gamma>0$. Previously, the algorithm by Chang, Pettie, and Zhang can construct a $(1/6,1/\text{poly}\log n)$-expander decomposition using $\tilde{O}(n^{1-\delta})$ rounds for any $\delta>0$, with a caveat that the algorithm is allowed to throw away a set of edges into an extra part which forms a subgraph with arboricity at most $n^{\delta}$. Our algorithm does not have this caveat. By slightly modifying the distributed algorithm for routing on expanders by Ghaffari, Kuhn and Su [PODC'17], we obtain a triangle enumeration algorithm using $\tilde{O}(n^{1/3})$ rounds. This matches the lower bound by Izumi and Le Gall [PODC'17] and Pandurangan, Robinson and Scquizzato [SPAA'18] of $\tilde{\Omega}(n^{1/3})$ which holds even in the CONGESTED CLIQUE model. This provides the first non-trivial example for a distributed problem that has essentially the same complexity (up to a polylogarithmic factor) in both CONGEST and CONGESTED CLIQUE. The key technique in our proof is the first distributed approximation algorithm for finding a low conductance cut that is as balanced as possible. Previous distributed sparse cut algorithms do not have this nearly most balanced guarantee.

==> Backup/SSS2.tex <==
\section{Nearly Most Balanced Sparse Cut} \label{XXX-sect-balanced-cut}

The goal of this section is to prove the following theorem.




\restatenearlybalcut*
\begin{proof}
This theorem follows from a re-parameterization of Lemma~\ref{XXX-lem-partition-nibble} and  Lemma~\ref{XXX-lem-partition-nibble-impl}.
\end{proof}

We will prove this theorem by adapting the nearly most balanced sparse cut algorithm of Spielman and Teng~\cite{SpielmanT13} to $\CONGEST$ in a white-box manner. Before presenting the proof, we highlight the major differences between this work and the sequential algorithm of~\cite{SpielmanT13}.
The procedure \nibble\ itself is not suitable for a distributed implementation, so we follow the idea of~\cite{ChangPZ19} to consider an approximate version of \nibble\  (Section~\ref{subsect-apx-nibble}) and use the distributed implementation described in~\cite{ChangPZ19} (Section~\ref{XXX-sect-partition-impl}).
The nearly most balanced sparse cut algorithm of Spielman and Teng~\cite{SpielmanT13}
involves doing  $\tilde{O}(|E|)$  iterations of \nibble\ with a random starting vertex  on the {\em remaining subgraph}. We will show that this sequential process can be partially parallelized at the cost of worsening the conductance guarantee by a polylogarithmic factor (Section~\ref{subsect-par-nibble}).



\paragraph{Terminology.} Given a parameter $\phi \in (0,1)$, We define the following functions as in~\cite{SpielmanT13}, where the values of the constants are $c_1 = 200$, $x_2 = 280$, $c_3 = 1800$, and $c_4 = 140$. The constant $c_4$ is used in the definition of \nibble.
\begin{align*}
    \ell &\bydef \ceil{\log(\vol(V))},\\
    \tlast &\bydef (\ell+1)\ceil{(2/\phi^2) \ln\left( c_1 (\ell+2) \sqrt{\vol(V) / 2}\right)},\\
    f_1(\phi) &\bydef \frac{1}{c_2(\ell+2) \tlast},\\
    \epsilon_b &\bydef 1/\left(c_3 (\ell+2) \tlast 2^b\right).
\end{align*}

Let $A$ be the adjacency matrix of the graph $G=(V,E)$.
We assume a 1-1 correspondence between $V$ and $\{1, \ldots, n\}$.
In a \textit{lazy random walk}, the walk stays at the current vertex with probability $1/2$ and otherwise moves to a random neighbor of the current vertex.
The matrix realizing this walk can be expressed as
 $M = (A D^{-1} + I) / 2$,
  where $D$ is the diagonal matrix with
  $(\deg(1), \ldots , \deg(n))$ on the diagonal.
  
Let $p_t^v$ be the probability distribution of the lazy random walk that begins at $v$ and walks for $t$ steps.
In the limit, as $t\rightarrow \infty$, 
$p_t(x)$ approaches $\deg(x)/2m$, so it is natural to measure 
$p_t(x)$ \emph{relative} to this baseline.
\[
\rho_t(x)=p_t(x)/\deg(x),
\]
%Define $\pi_t$ to be the permutation that sorts $V=\{1,\ldots,n\}$ in decreasing order of $\rho_t$-values, breaking ties by vertex ID. 

Let $p:  V \mapsto [0,1]$ be any function. 
The truncation operation $[p]_\epsilon$ 
rounds $p(x)$ to zero if it falls below a threshold that depends on $x$.
\[
  [p]_{\epsilon} (x)
=
\begin{cases}
  p (x) & \text{if $p (x) \geq \epsilon \deg(x)$,}\\
  0 & \text{otherwise}.
\end{cases}
\]
For each $1 \leq j \leq |V|$, we write $S_j(p)$ to denote the set of the top $j$ vertices with the highest $p(v)/\deg(v)$-value, breaking ties by comparing IDs. We also write $\lambda_j(p) = \vol(S_j)$.


As in~\cite{SpielmanT13}, for any vertex set $S$, we define the vector  $\chi_S$ by $\chi_S(u) = 1$ if $u \in S$ and $\chi_S(u) = 0$ if $u \notin S$, and we define the vector  $\psi_S$ by $\psi_S(u) = \deg(u) / \vol(S)$ if $u \in S$ and $\psi_S(u) = 0$ if $u \notin S$. In particular, $\chi_v$ is a probability distribution on $V$ that has all its probability mass on the vertex $v$, and $\psi_V$ is the degree distribution of $V$. 

\subsection{Nibble}
We first review the \nibble\ algorithm of~\cite{SpielmanT13}, which computes the following two sequences of vectors with truncation parameter $\epsilon_b$.
\begin{align*}
q_t &=\begin{cases}
\chi_v & \text{if $t = 0$,}\\
M r_{t-1} & \text{otherwise.}
\end{cases}\\
r_t & = [q_t]_{\epsilon_b}.
\end{align*}
We note that the following is true for all $u \in V$ and $t \geq 0$.
\[p_t(u) \geq q_t(u) \geq r_t(u).\]


\begin{framed}
\noindent {\bf Algorithm} \nibble($G,v,\phi,b$)

\medskip

For $t  = 1$ to $\tlast$, if there exists an index $1 \leq j \leq |V|$ meeting the following four conditions 
\begin{enumerate}
\addtolength{\itemindent}{1cm}
    \item[(C.1)] $\Phi(S_j(q_t)) \leq \phi$.
    \item[(C.2)] $\lambda_j(q_t) \leq (5/6) \vol(V)$.
    \item[(C.3)] $2^b \leq \lambda_j(q_t)$. 
    \item[(C.4)] Let $j^\ast$ be the smallest index such that $2^b \leq \lambda_{j^\ast}(q_t)$. Then $q_t(u) / \deg(u) \geq \frac{1}{c_4 (\ell+2) 2^b}$ for each  $u \in S_{j^\ast}(q_t)$.
\end{enumerate}
then return $C = S_j(q_t)$ and quit.
Otherwise return $C = \emptyset$.
\end{framed}

Note that the definition of \nibble($G,v,\phi,b$) is exactly the same as the one presented in~\cite{SpielmanT13}. In~\cite{SpielmanT13}, (C.4) is written alternatively and equivalently as $I_x(q_t, 2^b) \geq \frac{1}{c_4 (\ell+2) 2^b}$. 


\begin{definition}
 Define $Z_{u,\phi,b}$ as the subset of $V$ such that if we start the lazy random walk from $v \in Z_{u,\phi,b}$, then $\rho_t(u) \geq \epsilon_b$ for at least one of  $t \in [0, \tlast]$. 
 For any edge $e = \{u_1, u_2\}$, define $Z_{e, \phi, b} = Z_{u_1,\phi,b} \cup Z_{u_2,\phi,b}$.
 \end{definition}
 
 Intuitively, if $v \notin Z_{e, \phi, b}$, then $e$ does not  participate in \nibble($G,v,\phi,b$). Note that $v \in Z_{e, \phi, b}$ is  a necessary but not sufficient condition for $e \in E(C)$, where $C$ is the output of \nibble($G,v,\phi,b$).
The following auxiliary lemma establishes upper bounds on $\vol(Z_{u,\phi,b})$ and $\vol(Z_{e,\phi,b})$. This lemma will be applied to bound the amount of congestion when we execute multiple \nibble\ in parallel. Intuitively, if $\vol(Z_{e,\phi,b})$ is small, then we can afford to run many instances \nibble($G,v,\phi,b$) in parallel for random starting vertices $v$ sampled from the degree distribution $\psi_V$.

\begin{lemma}\label{XXX-lem-nibble-aux}
The following formulas hold for each vertex $u$ and each edge $e$.
\begin{align*}
    &\vol(Z_{u,\phi,b}) \leq (\tlast+1) / \epsilon_b\\
    &\vol(Z_{e,\phi,b}) \leq 2(\tlast+1) / \epsilon_b
\end{align*}
In particular, these two quantities are both upper bounded by $3 c_3 \tlast^2 \ell 2^b = O\left(\frac{ 2^b  \log^5 \vol(V)}{\phi^4}\right)$.
\end{lemma}
\begin{proof}
In this proof we use superscript to indicate the starting vertex of the lazy random walk.
We write $Z_{u,\phi,b,t} = \{ v \in V \ | \ \rho_t^v(u) \geq \epsilon_b \}$. Then $\vol(Z_{u,\phi,b}) \leq \sum_{t = 0}^{\tlast} \vol(Z_{u,\phi,b,t})$. Thus, to prove the lemma, if suffices to show that $\vol(Z_{u,\phi,b,t}) \leq 1 / \epsilon_b$.
This inequality follows from the fact that $\rho_t^v(u) = \rho_t^u(v)$, as follows.
\begin{align*}
1 &= \sum_{v \in V} p_t^u(v) \\
&\geq  \sum_{v \in V \ | \ \rho_t^u(v) \geq \epsilon_b} p_t^u(v) \\
&\geq \sum_{v \in V \ | \ \rho_t^u(v) \geq \epsilon_b} \epsilon_b \cdot \deg(v) \\
&= \sum_{v \in V \ | \ \rho_t^v(u) \geq \epsilon_b} \epsilon_b \cdot \deg(v) \\
&= \epsilon_b \cdot  \vol(Z_{u,\phi,b,t}).
\end{align*}
The fact that $\rho_t^v(u) = \rho_t^u(v)$ as been observed in~\cite{SpielmanT13} without a proof. 
For the sake of completeness, we will show a proof of this fact. An alternate proof can be found in~\cite[Lemma 3.7]{ChangPZ19}. In the following calculation, we use the fact that $D^{-1} M D = D^{-1}(AD^{-1}+I)D/2 = (D^{-1}A + I)/2 =  M^{\top}$.
\begin{align*}
    \rho_t^v(u) &= \chi_u^\top D^{-1} M^t \chi_v\\
    &= \chi_u^\top (D^{-1} M D)^t   (D^{-1}\chi_v)\\
    &= \chi_u^\top (M^{\top})^t   (D^{-1}\chi_v)\\
    &=  (D^{-1}\chi_v)^\top M^t \chi_u \\
    &=  \chi_v^\top D^{-1}  M^t \chi_u \\
    &= \rho_t^u(v).
\end{align*}
Finally, recall that $\epsilon_b = 1/\left(c_3 (\ell+2) \tlast 2^b\right)$, and so 
$2(\tlast + 1)/\epsilon_b =  2(\tlast + 1) \cdot c_3 (\ell+2) \tlast 2^b <  3 c_3 \tlast^2 \ell 2^b$. We assume that $\vol(V)$ is at least a sufficiently large constant so that the above calculation holds.
\end{proof}

 Lemma~\ref{XXX-lem-nibble} lists some crucial properties of \nibble.   In subsequent discussion, for any given subset $S\subset V$, the subset $S^g \subseteq S$ and the partition $S^g = \bigcup_{b=1}^{\ell} S^g_b$  are defined according to Lemma~\ref{XXX-lem-nibble}. 
 

\begin{lemma}[Analysis of \nibble]\label{XXX-lem-nibble}
For each $\phi \in (0,1]$, and for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi),
\end{align*}
there exists a subset $S^g \subseteq S$ with the following properties.
First, $\vol(S^g)\geq \vol(S)/2$.  Second, $S^g$ is partitioned into
$S^g = \bigcup_{b=1}^{\ell} S^g_b$ such that if a lazy random walk is initiated
at any $v\in S^g_b$ with truncation parameter
$\epsilon_b$, the following are true.
\begin{enumerate}
    \item\label{XXX-N1} The set $C$ returned by \nibble$(G,v,\phi,b)$ is non-empty.
    \item\label{XXX-N2} 
    Let $1 \leq t \leq  \tlast$, and let $j^\ast$ be the smallest index such that $2^b \leq \lambda_{j^\ast}(q_t)$. If    $q_t(u) / \deg(u) \geq \frac{1}{c_4 (\ell+2) 2^b}$ for each  $u \in S_{j^\ast}(q_t)$, then  $\vol(S_{j^\ast}(q_t) \cap S) \geq 2^{b-1}$.
\end{enumerate}
\end{lemma}
\begin{proof}
The first condition follows from~\cite[Theorem 2.1 (N.3)]{SpielmanT13}. The second condition follows from the proof of~\cite[Lemma 2.8]{SpielmanT13}. 
\end{proof}

To put it another way, Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N1}) says that there exist  $1 \leq t \leq  \tlast$ and $1 \leq j \leq |V|$ such that (C.1)--(C.4) are met;   Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N2}) says that for any choice of  $1 \leq t \leq  \tlast$   satisfying (C.4), we have $\vol(S_{j^\ast}(q_t) \cap S) \geq 2^{b-1}$, where $j^\ast$ is the index considered in (C.4).

Intuitively, the set $S^g$ represents the ``core'' of $S$ in the sense that \nibble$(G,v,\phi,b)$  is guaranteed to return a  sparse cut $C$ if $v \in S_b^g$. Recall that (C.1) and (C.2) in the description of \nibble$(G,v,\phi,b)$ guarantees that the cut $C$ has conductance at most $\phi$ and has volume at most $(5/6)\vol(V)$. 

\subsection{Approximate Nibble}\label{subsect-apx-nibble}
The  algorithm \nibble\ is not suitable for a distributed implementation since it has to go over all possible $j$. Similar to the idea of~\cite[Algorithm~1]{ChangPZ19} we provide a slightly modified version of \nibble\ that only considers $O((1/\phi)\log n)$ choices of $j$ for each $t$.
The cost of doing so is that we have to relax the two conditions (C.1) and (C.2) slightly.

\begin{framed}
\noindent {\bf Algorithm} \distnibble($G,v,\phi,b$)

\medskip

For $t  = 1$ to $\tlast$, and for $x = 0$ to $\floor{\log_{1+\phi} (5/6)\vol(V)}$, set  $j$ as the smallest index such that $\vol(S_j(q_t)) \geq (1+\phi)^x$. If the parameter $j$ meets the following four conditions
\begin{enumerate}
\addtolength{\itemindent}{1cm}
    \item[(C.1*)] $\Phi(S_j(q_t)) \leq 12\phi$.
    \item[(C.2*)] $\lambda_j(q_t) \leq (11/12) \vol(V)$.
    \item[(C.3)] $2^b \leq \lambda_j(q_t)$.
    \item[(C.4)] Let $j^\ast$ be the smallest index such that $2^b \leq \lambda_{j^\ast}(q_t)$. Then $q_t(u) / \deg(u) \geq \frac{1}{c_4 (\ell+2) 2^b}$ for each  $u \in S_{j^\ast}(q_t)$.
\end{enumerate}
then return $C = S_j(q_t)$ and quit.
Otherwise return $C = \emptyset$.
\end{framed}



\begin{definition}\label{def-participate-edges}
Consider \distnibble$(G,v,\phi,b)$. Define $P^\ast$ as the set of edges  $e$ such that there exist at least one endpoint $u$ of $e$ and at least one number $t \in [0, \tlast - 1]$ with $r_t(u) > 0$.
\end{definition}

 Intuitively,   $P^\ast$  is the set of edges that participate in   \distnibble($G,v,\phi,b$). This notation will be used in analyzing the complexity of our distributed implementation.


%\begin{definition}
%Consider \distnibble$(G,v,\phi,b)$. 
%If the output $C$ is non-empty, then define $C^\ast = \{ u \in C \ | \ \rho_t(u) \geq \epsilon_b \}$, where $t$ is the index such that $C = S_j(q_t)$; otherwise define  $C^\ast = \emptyset$.
%\end{definition}

%Due to the facts that $\epsilon_b < \frac{1}{c_4 (\ell+2) 2^b}$ and $\rho_t(u) = p_t(u)/\deg(u) \geq q_t(u)/\deg(u)$, we always have $S_{j^\ast}(q_t) \subseteq C^\ast$, where $j^\ast$ is the index considered in (C.4), for the case the output $C$ is non-empty.

Regardless of the choice of $b$ and $v$, the output $C$ of \distnibble$(G,v,\phi,b)$ must satisfy $\Phi(C) \leq 12\phi$ and   $\vol(C) \leq (11/12) \vol(V)$. Lemma~\ref{XXX-lem-dist-nibble} shows an additional property of $C$ when $v$ is appropriately chosen.

\begin{lemma}[Analysis of \distnibble]\label{XXX-lem-dist-nibble}
For each $0 < \phi \leq 1/12$, and for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi),
\end{align*}
the output $C$ of \distnibble$(G,v,\phi,b)$ for any $v \in S_g^b$ is non-empty and it satisfies 
\[\vol(C \cap S) %\geq \vol(C^\ast \cap S)  
\geq 2^{b-1}.\]
\end{lemma}
\begin{proof}
We pick $(t,j)$ as the indices that satisfy (C.1)--(C.4), whose existence is guaranteed by Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N1}). Let $v \in S_g^b$. We first show that the output $C$ of \distnibble$(G,v,\phi,b)$ is non-empty. That is, we argue that there exists an index $j' \geq j$ such that the pair  $(t,j')$ is under consideration in \distnibble($G,v,\phi,b$) and it satisfies all four conditions (C.1*), (C.2*), (C.3), and (C.4). 
Remember that an index $j'$ is under consideration in 
\distnibble($G,v,\phi,b$) if there exists an integer $x$ within the range $[0, \log_{1+\phi} (5/6)\vol(V)]$ such that $j'$ is the smallest index satisfying  $\vol(S_{j'}(q_t)) \geq (1+\phi)^x$. 
Specifically, we select $j'$  as the smallest index such that $j' \geq j$ and $j'$ is considered in \distnibble($G,v,\phi,b$).
Since $t$ is fixed, from now on we write $S_j$ as a shorthand for  $S_j(q_t)$, and $S_{j'}$ for $S_{j'}(q_t)$.  


\paragraph{Conditions (C.1*) and (C.2*).} We first verify that (C.1*) and (C.2*) are met. We divide the analysis into two cases.
\begin{itemize}
\item Consider the case $\vol(S_{j'}) \leq \vol(V)/2$. We have $|\partial(S_{j'})| \leq |\partial(S_j)| + \phi \vol(S_j) \leq 2\phi \vol(S_j) \leq 2\phi \vol(S_{j'})$, and so $\Phi(S_{j'}) = |\partial(S_{j'})| / \vol(S_{j'}) \leq 2\phi$, and so (C.1*) is met.
In the above calculation, we use the fact that $|\partial(S_j)| \leq \phi \vol(S_j)$, which is due to the assumption that  $(t,j)$ satisfies (C.1).
Note that (C.2*) is automatically met in this case.


\item Consider the case $\vol(S_{j'}) > \vol(V)/2$.
The following calculation shows that (C.2*) is met. The calculation uses the facts that $\phi \leq 1/12$ and $\vol(V \setminus S_{j}) \geq (1/6)\vol(V)$, where the latter is due to the assumption that  $(t,j)$ satisfies (C.2).
\begin{align*}
    \vol(V \setminus S_{j'}) &\geq
    \vol(V \setminus S_{j}) - \phi \vol(S_j) \\
    &\geq \vol(V \setminus S_{j}) - (1/12)\vol(S_j)\\
    &\geq \vol(V \setminus S_{j}) - (1/12)\vol(V)\\
    &\geq \vol(V \setminus S_{j}) / 2\\
    &\geq (1/12)\vol(V).
\end{align*}
Similarly, we have $|\partial(S_j')| \leq \phi \vol(V \setminus S_{j}) + \phi \vol(S_j)$. 
Since $\vol(S_{j}) \leq (5/6)\vol(V)$, we have $\phi \vol(S_j) \leq 5 \phi \vol(V \setminus S_j)$.
Therefore, $|\partial(S_j')| \leq 6\phi \vol(V \setminus S_{j}) \leq 12\phi  \vol(V \setminus S_{j'})$, which implies  (C.1*).
\end{itemize}


\paragraph{Conditions (C.3)  and (C.4).}
We also observe that (C.3)  and (C.4) also hold for the parameters $(t,j')$, as follows. Remember that (C.3)  and (C.4) hold for the parameters $(t,j)$. Since $\lambda_{j'}(q_t) > \lambda_{j}(q_t)$ so long as $j' > j$, we infer that (C.3) also holds for  $(t,j')$.  Also,  (C.4) automatically holds for  $(t,j')$ since this condition only depends on $t$.


\paragraph{Lower Bound of $\vol(C\cap S)$.}
Finally, we prove that $\vol(C \cap S) \geq 2^{b-1}$.
Select $j^\ast$ as the index considered in (C.4). Note that we must have $j^\ast \leq j \leq j'$, and so
%By definition of $C^\ast$, we have 
  $S_{j^\ast} \subseteq  S_j \subseteq S_{j'} = C$.  Therefore, all we need to do is to show that $\vol(S_{j^\ast} \cap S) \geq 2^{b-1}$.
This follows from Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N2}) and the fact that $t$ satisfies (C.4).
\end{proof}

Lemma~\ref{XXX-lem-dist-nibble} shows that if $v \in S_g^b$, then the output $C$ of \distnibble$(G,v,\phi,b)$ is non-empty, and so it has conductance at most $12 \phi$ and volume at most $(11/12)\vol(V)$ in view of (C.1*) and (C.2*). 

Recall that the main goal of Section~\ref{XXX-sect-balanced-cut} is to design a distributed algorithm that finds a nearly most balanced sparse cut, so finding a cut $C$ satisfying (C.1*) and (C.2*) is not enough. This is in contrast to~\cite{ChangPZ19}, where they do not need the output cut to satisfy any balance constraint.

Following the approach of~\cite{SpielmanT13}, to find a nearly most balanced sparse cut, we will need to take the union of the output of multiple instances of \distnibble, and the goal of the analysis is to show that the resulting vertex set has volume at least $\vol(S)/2$.  
This explains the reason why we not only need to show that $C \neq \emptyset$ but also  need to show a lower bound of $\vol(C \cap S)$ in Lemma~\ref{XXX-lem-dist-nibble}.





\subsection{Random Nibble}\label{subsect-rnd-nibble}
Note that both \nibble\ and \distnibble\ are deterministic. Next, we consider the algorithm \randnibble\ which executes \distnibble\ with a random starting vertex $v$ and a random parameter $b$. The definition of  \randnibble\ exactly the same as the corresponding one in~\cite{SpielmanT13} except that we use \distnibble\ instead of \nibble.


\begin{framed}
\noindent {\bf Algorithm} \randnibble($G,\phi$)

\medskip

Sample a starting vertex $v \sim \psi_V$ according to the degree distribution. Choose a number $b \in [1, \ell]$ with $\Prob[b = i] = 2^{-i} / (1 - 2^{-\ell})$. Execute \distnibble($G,v,\phi,b$), and return the result $C$.
\end{framed}

The set of edges $P^\ast$ (Definition~\ref{def-participate-edges}) participating in the subroutine \distnibble($G,v,\phi,b$) satisfies that $P^\ast \subseteq E(C)$, where $C$ is the output of  \randnibble($G,\phi$). Therefore, Lemma~\ref{XXX-lem-rand-nibble} also implies that  $\Prob[e \in E(C)] \leq (4 c_3 \tlast^2 \ell^2) /\vol(V)$ for each $e \in E$.



\begin{lemma}[Analysis of \randnibble]\label{XXX-lem-rand-nibble}
For each $0 < \phi \leq 1/12$, the following holds for the output $C$ of \distnibble$(G,v,\phi,b)$. 
\begin{enumerate}
    \item  $\Prob[e \in P^\ast] \leq (4 c_3 \tlast^2 \ell^2) /\vol(V)$ for each $e \in E$, where $P^\ast$ is the set of edges participating in the subroutine \distnibble$(G,v,\phi,b)$.
   % \item $\Prob[u \in C^\ast] \leq  (4 c_3 \tlast^2 \ell^2) /\vol(V)$ for each $u \in V$.
    \item  $\Expect[\vol(C \cap S)]
    %\geq \Expect[\vol(C^\ast \cap S)] 
    \geq \frac{\vol(S)}{4 \vol(V)}$ for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi).
\end{align*} 
\end{enumerate}
\end{lemma}
\begin{proof}
The proof of $\Expect[\vol(C  \cap S)] \geq \frac{\vol(S)}{4 \vol(V)}$ follows from Lemma~\ref{XXX-lem-dist-nibble}  and the proof of~\cite[Lemma 3.1]{SpielmanT13}. An upper bound of $\Prob[e \in P^\ast]$ can be calculated using Lemma~\ref{XXX-lem-nibble-aux}. More specifically, observe that $v \in Z_{e,\phi,i}$ is a necessary condition for $e \in E(C)$ for the case $b = i$, and so we can upper bound $\Prob[e \in P^\ast]$ as follows.
\begin{align*}
    \Prob[e \in P^\ast] &\leq \sum_{i=1}^{\ell} \Prob[b = i] \cdot \vol(Z_{e,\phi,i}) / \vol(V)\\
    &\leq \sum_{i=1}^{\ell} \frac{2^{-i}}{1 - 2^{-\ell}} \cdot  (3 c_3 \tlast^2 \ell 2^i) /\vol(V)\\
    &< \sum_{i=1}^{\ell} (4 c_3 \tlast^2 \ell) /\vol(V)\\
    &=  (4 c_3 \tlast^2 \ell^2) /\vol(V). \qedhere
\end{align*}
%The calculation of $\Prob[u \in C^\ast]$ is similar, as we observe that $v \in Z_{u,\phi,i}$ is a necessary condition for $u \in C^\ast$ for the case $b = i$.
\end{proof}


%Lemma~\ref{XXX-lem-rand-nibble}(2) and Lemma~\ref{XXX-lem-rand-nibble}(3) will be crucial when we analyze the intersection of $S$ and the vertex set resulting from combining the output of multiple instances of \randnibble($G,\phi$).
%The proof of Lemma~\ref{XXX-lem-rand-nibble} explains the technical reason as to why we consider $C^\ast$ instead of $C$. The proof of the upper bound of $\Prob[u \in C^\ast]$ in  Lemma~\ref{XXX-lem-rand-nibble} does not hold if we replace $C^\ast$ with $C$. In principle, the set $C=S_j(q_t)$ might include vertices $u$ with very small $\rho_t(u)$-value. 
%For comparison, the analysis of~\cite{SpielmanT13} does not suffer from this issue since in their algorithm \randnibble($G,\phi$) is applied \emph{sequentially}, not  \emph{in parallel}. 


\subsection{Parallel Nibble} \label{subsect-par-nibble}
In~\cite{SpielmanT13}, roughly speaking, it was shown that a nearly most balanced sparse cut can be found with probability $1 - p$ by \emph{sequentially} applying \nibble\ with a random starting vertex for $O(|E| \log (1/p))$ times.
After each \nibble, the output subset $C$ is removed from the underlying graph. To achieve an efficient implementation in $\CONGEST$, we need to diverge from this approach and aim at doing multiple \distnibble\ \emph{in parallel}. 

However, the na\"{i}ve approach of doing all $O(|E| \log (1/p))$ \randnibble\ in parallel does not work, since the potentially high overlap between the output subsets of different execution of \randnibble\ will destroy the required conductance constraint.

In what follows, we consider the algorithm \parallelnibble, which involves a simultaneous execution of a moderate number of \distnibble.
In the description of \parallelnibble, we say that $e$ participates in the subroutine \randnibble($G,\phi$) if $e \in P^\ast$ for the subroutine \distnibble($G,v,\phi,b$) during the execution of \randnibble($G,\phi$).

\begin{framed}
\noindent {\bf Algorithm} \parallelnibble($G, \phi$)

\medskip

For $i = 1$ to $k \bydef \ceil{\vol(V) / (4 c_3 \tlast^2 \ell^2)}$, do \randnibble($G,\phi$), in parallel. Let $C_i$ be the result of the $i$th execution of \randnibble($G,\phi$). Let $U_i = \bigcup_{j=1}^i C_i$.  If there exists an edge $e$ participating in the subroutine \randnibble($G,\phi$) for more than $w \bydef 10 \ceil{\ln (\vol(V))}$ times, return $C = \emptyset$.
Otherwise select $i^\ast \in [1, k]$ to be the highest index such that $\vol(U_{i^\ast}) \leq z  \bydef (23/24)\vol(V)$. Return $C = U_{i^\ast}$.
\end{framed}

For the sake of presentation, in the statement of Lemma~\ref{XXX-lem-par-nibble} we define the function $g$ by
\[g(\phi, \vol(V)) \bydef 20 c_3 w \tlast^2  \ell^2.\]
In particular, we have $5w \vol(V)/k \leq g(\phi, \vol(V))$. The function $g$ will also be used in the description and the analysis of \balancedcut\ in the subsequent discussion. 
 
\begin{lemma}[Analysis of \parallelnibble]\label{XXX-lem-par-nibble}
For each $0 < \phi \leq 1/12$ 
the following is true for the output $C$ of \parallelnibble$(G, \phi)$.
\begin{enumerate}
    \item If $C \neq \emptyset$, then  $\Phi(C) \leq 552 w \phi$. 
    \item For each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi),
\end{align*} define the random variable $y$ as follows.
\[
y = 
\begin{cases}
\vol(S), \text{ if } \vol(C) \geq (1/24)\vol(V) \\
\vol(C \cap S), \text{ otherwise}\\
\end{cases}
\]
Then $\Expect[y] \geq \frac{k \vol(S)}{5w \vol(V)} \geq \frac{\vol(S)}{g(\phi, \vol(V))}$.
\end{enumerate}
\end{lemma}
\begin{proof}
We show that if the output subset $C$ is non-empty, then we must have $\Phi(C) \leq 552 w \phi$. 
By definition of \parallelnibble, if the output is non-empty, then each edge $e$ is included in at most $w$ of these subsets $E(C_1), \ldots, E(C_{i^\ast})$. Therefore, 
\begin{align*}
 \vol(C) &\geq (1/w)  \sum_{i=1}^{i^\ast} 2 |E(C_i)| \\
 &\geq   (1/w)   \sum_{i=1}^{i^\ast} \vol(C_i) /  (1 + 12\phi)\\
 &\geq \frac{1}{2w} \sum_{i=1}^{i^\ast} \vol(C_i).
\end{align*}
%$\vol(C) \geq (1/w) \sum_{i=1}^{i^\ast} \vol(C_i)$. 
Using the fact that the output $C_i$ of \distnibble$(G,v,\phi,b)$ has $\Phi(C_i)\leq 12\phi$ and the above calculation, we upper bound $|\partial(C)|$ as follows.
\begin{align*}
    |\partial(C)| &\leq \sum_{i=1}^{i^\ast} |\partial(C_i)|\\ &\leq  \sum_{i=1}^{i^\ast} 12 \phi \vol(C_i)\\
    &\leq 24w \phi \vol(C).
\end{align*}
The threshold $z$ guarantees that $\vol(V \setminus C) \geq (1/23) \vol(C)$, and so $|\partial(C)|  \leq  24 \cdot 23 \cdot w \phi \vol(V \setminus C) = 552 w \phi \vol(V \setminus C)$. We conclude that $\Phi(C) \leq 552 w \phi$. 



Next, we analyze the random variable $y$. We first observe that if $i^\ast <  k$, then $C = U_{i^\ast}$ has $\vol(C) \geq (1/24) \vol(V)$.
This is because that each $C_i$ must have $\vol(C_i) \leq (11/12) \vol(V)$ by definition of \distnibble. 
If $\vol(U_{i^\ast}) < (1/24) \vol(V)$, then $\vol(U_{i^\ast + 1}) <   (1/24) \vol(V) +  (11/12) \vol(V) <  (23/24) \vol(V)$, contradicting the choice of $i^\ast$.
Thus, for the case $i^\ast <  k$, we automatically have $y = \vol(S)$, which is the maximum possible value of $y$. In view of this, we can lower bound $\Expect[y]$ as follows.
\[
\Expect[y] \geq \Expect[\vol(U_k \cap S)] - \Prob[B] \cdot \vol(S),
\]
where $B$ is the  event that there exists an edge  participating in the subroutine \randnibble($G,\phi$) for more than $w$ times.
Note that $B$ implies $C = \emptyset$, but not vise versa.

By Lemma~\ref{XXX-lem-rand-nibble}, we know that $\Expect[\vol(C_i \cap S)] \geq \frac{\vol(S)}{4 \vol(V)}$, and this implies $\Expect[\vol(U_k \cap S)] \geq (1/w) \sum_{i=1}^{k} \Expect[\vol(C_i)] = \frac{k\vol(S)}{4w \vol(V)}$.
Therefore, to obtain the desired bound $\Expect[y] \geq \frac{k\vol(S)}{5w \vol(V)}$, it remains to show that $\Prob[B] \leq \frac{k}{20w \vol(V)}$.


If $k = 1 \leq w$, then $\Prob[B] = 0$.
In what follows, we assume $k \geq 2$, and this implies
$k \leq 2 \cdot \vol(V) / (4 c_3 \tlast^2 \ell^2)$.
Let $e \in E$. Define $X_i = 1$ if $e$ participates in the $i$th \randnibble($G,\phi$), and define $X_i = 0$ otherwise. Set  $X = \sum_{i=1}^k X_i$.
By Lemma~\ref{XXX-lem-rand-nibble} and the inequality $k \leq 2 \cdot \vol(V) / (4 c_3 \tlast^2 \ell^2)$, we infer that $\Expect[X] \leq 2$. By a Chernoff bound, $\Prob[X > w] \leq \exp(- 2(w-2) / 3) \ll (\vol(V))^{-2}$. By a union bound over all edges $e \in E$, we infer that $\Prob[B] < (\vol(V))^{-1} \ll \frac{k}{20w \vol(V)}$, as required.
\end{proof}


Intuitively, Lemma~\ref{XXX-lem-par-nibble} shows that we only lose a factor of $O(\log n)$ in conductance if we combine the result of $k$ parallel executions of \randnibble($G,\phi$).
We are now ready to present the algorithm for finding a nearly most balanced sparse cut, which involves executing \parallelnibble\ sequentially for $s = O(\poly(1/\phi, \log n))$ times on the remaining subgraph.


\begin{framed}
\noindent {\bf Algorithm} \balancedcut($G, \phi, p$)

\medskip
 Initialize $W_0 = V$. For $i = 1$ to $s \bydef 4 g(\phi, \vol(V)) \ceil{\log_{7/4}(1/p)}$ do the following.
\begin{enumerate}
    \item Execute \parallelnibble($G\{W_{i-1}\}, \phi$). Let the output be $C_i$. 
    \item Set $W_i = W_{i-1} \setminus C_i$. 
    \item If $\vol(W_i) \leq (47/48)\vol(V)$ or $i=s$, return $C = \bigcup_{j=1}^i C_j$ and quit.
\end{enumerate}
\end{framed}


\begin{lemma}[Analysis of \balancedcut]\label{XXX-lem-partition-nibble}
Let $C$ be the output of \balancedcut($G, \phi$), with  $0 <  \phi \leq 1/12$.
Then the following holds:
\begin{enumerate}
\item \label{XXX-P1} $\vol(C) \leq (47/48) \vol(V)$.
\item \label{XXX-P2} If $C \neq \emptyset$, then $\Phi(C) =  O(\phi \log |V|)$.
\item \label{XXX-P3} Furthermore, 
for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{1}{2} \cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi) / 2,
\end{align*}
with probability at least $1-p$, at least one of the following holds:
\begin{enumerate}
    \item \label{XXX-P3a} $\vol(C) \geq (1/48)\vol(V)$.
    \item \label{XXX-P3b} $\vol(S \cap C) \geq (1/2) \vol(S)$.
\end{enumerate}
\end{enumerate}
\end{lemma}
\begin{proof} This proof follows the framework of~\cite[Theorem 3.2]{SpielmanT13}.

\paragraph{Proof of Condition~\ref{XXX-P1}.} 
Let $i'$ be the index such that the output subset $C$ is $\bigcup_{j=1}^{i'} C_j$. Then we have $\vol(C) \leq \vol(V \setminus W_{i'-1}) + \vol(C_{i'})$.
Since the algorithm does not terminate at the $(i'-1)$th iteration, we have $\vol(W_{i'-1}) > (47/48)\vol(V)$, and so
$\vol(V \setminus W_{i'-1}) \leq (1/48)\vol(V)$.
By the algorithm description of \parallelnibble, we have  $\vol(C_{i'}) \leq (23/24)\vol(W_{i'-1}) \leq (23/24)\vol(V)$. To summarize, we have $\vol(C) \leq (1/48)\vol(V) + (23/24)\vol(V) = (47/48)\vol(V)$.

\paragraph{Proof of Condition~\ref{XXX-P2}.} 
Note that the sets $C_1, \ldots, C_{i'}$ that constitute
 $C = \bigcup_{j=1}^{i'} C_j$ are disjoint vertex sets.
 We have $|\partial(C)| \leq \sum_{j=1}^{i'} |\partial(C_i)| \leq O(\phi \log |V|) \sum_{j=1}^{i'} \vol(C_i) =  O(\phi \log |V|) \cdot \vol(C)$, where the second inequality is due to Lemma~\ref{XXX-lem-par-nibble}.
 By Condition~\ref{XXX-P1}, we infer that $\vol(V \setminus C) \geq (1/48) \vol(C)$, and so we also have $|\partial(C)| \leq O(\phi \log |V|) \cdot \vol(V \setminus C)$. Hence $\Phi(C) = O(\phi \log |V|)$.


\paragraph{Proof of Condition~\ref{XXX-P3}.} 
 We focus on $h \bydef 4g(\phi, \vol(V))$ consecutive iterations from $i = x+1$ to  $i = x+h$, for some index $x$.
For each index $j \in [1, h]$, we write $H_j$ to denote  the event that (1) $\vol(S \cap W_{x+j-1}) \leq \vol(S)/2$ or (2) the algorithm ends prior to iteration $i = x+j$. 
We define the random variable $Y_j$ as follows. 
\[
Y_j = 
\begin{cases}
\frac{\vol(S)}{2g(\phi, \vol(V))} &\text{ if $H_j$ occurs (Case 1)} \\
\vol(W_{x+j-1} \cap S) &\text{ if } \vol(C_{x+j}) \geq (1/24)\vol(W_{x+j-1}) \text{ (Case 2)} \\
\vol(C_{x+j} \cap S) &\text{ otherwise (Case 3)}\\
\end{cases}
\]
We  claim that if $H_j$ does not occur, then the preconditions of Lemma~\ref{XXX-lem-par-nibble} are  met for the cut $S' = S \cap W_{x+j-1}$ in the graph $G' = G\{ W_{x+j-1}\}$ when we run \parallelnibble($G\{W_{x+j-1}\}, \phi$) during the $(x+j)$th iteration.
\begin{itemize}
\item We show that $\vol(S \cap W_{x+j-1}) \leq (2/3) \vol(W_{x+j-1})$, as follows. 

\begin{align*}
  \vol(S \cap W_{x+j-1}) 
  &\leq (1/2) \vol(V)  &\vol(S) \leq \vol(V)/2\\
  &< (1/2)(48/47) \vol(W_{x+j-1}) &\vol(W_{x+j-1}) > (47/48) \vol(V)\\
  &< (2/3) \vol(W_{x+j-1}).
\end{align*}

\item We show that  $\Psi_{G\{ W_{x+j-1}\}}(S) \leq 2\Phi(S) \leq f_1(\phi, \vol(V)) \leq f_1(\phi, \vol(W_{x+j-1}))$, where we write $f_1(\phi, r)$ to indicate the value of $f_1(\phi)$ when the underlying graph has volume $r$.

\begin{align*}
  \Psi_{G\{ W_{x+j-1}\}}(S)
  &= \frac{|E(S\cap W_{x+j-1},  W_{x+j-1} \setminus S)|}{\min\{\vol(S\cap W_{x+j-1}),\vol(W_{x+j-1} \setminus S)\}}\\
  &\leq \frac{|E(S, V \setminus S)|}{\min\{\vol(S\cap W_{x+j-1}),\vol(W_{x+j-1} \setminus S)\}}\\
  &< \frac{|E(S, V \setminus S)|}{(1/2)\min\{\vol(S),\vol(V \setminus S)\}}\\
  &= 2\Phi(S).
\end{align*}
  
The second inequality is explained as follows.
We have $\vol(S \cap W_{x+j-1}) > \vol(S)/2$ since $H_j$ does not occur, and we also have

\begin{align*}
\vol(W_{x+j-1} \setminus S) &\geq \vol(V \setminus S) - (1/48)\vol(V)\\
&\geq \vol(V \setminus S) - (1/24)\vol(V \setminus S) &\vol(V \setminus S) \geq (1/2)\vol(V)\\
&> \vol(V \setminus S)/2.
\end{align*}
\end{itemize}
Thus, we are able to use Lemma~\ref{XXX-lem-par-nibble} to infer that   that \[\Expect[Y_j \ | \ \overline{H_j}] \geq \frac{\vol(S \cap W_{x+j-1})}{g(\phi, \vol(W_{x+j-1}))} > \frac{\vol(S)}{2g(\phi, \vol(V))}.\]
In the calculation we use the two inequalities $g(\phi, \vol(V)) \geq g(\phi, \vol(W_{x+j-1}))$ and $\vol(S \cap W_{x+j-1}) > \vol(S)/2$, where the latter is due to $\overline{H_j}$.
Combining $\Expect[Y_j \ | \ \overline{H_j}] > \frac{\vol(S)}{2g(\phi, \vol(V))}$ with the trivial bound  $\Expect[Y_j \ | \ {H_j}] =  \frac{\vol(S)}{2g(\phi, \vol(V))}$, we conclude that
 \[\Expect[Y_j] \geq \frac{\vol(S)}{2g(\phi, \vol(V))}.\] 
 
We write $Y = \sum_{j=1}^h Y_j$, and we have  $\Expect[Y] \geq 2 \vol(S)$ in view of the above, as we recall $h = 4g(\phi, \vol(V))$.
We claim that we always have $Y \leq 4\vol(S)$.
We may write $Y = Y^1 + Y^2 + Y^3$, where $Y^i$ considers the part of $Y$ due to Case~$i$ in the definition of $Y_j$. It is clear that $Y^1 \leq h \cdot \frac{\vol(S)}{2g(\phi, \vol(V))} = 2 \vol(S)$. We claim that  $Y^2 \leq \vol(S)$ by observing that Case~2 can only occur at most once.  Suppose Case~2  occurs at iteration $i = x+j$. Then $\vol(C_{x+j}) \geq
(1/24)\vol(W_{x+j-1}) > (1/48)\vol(W_{x+j-1})$, which implies $\vol(W_{x+j}) \leq (47/48)\vol(W_{x+j-1}) \leq  (47/48)\vol(V)$, and so the algorithm terminates.  For Case~3, we have $Y^3 \leq \sum_{j=1}^h \vol(C_{x+j} \cap S) \leq \vol(S)$.
In view of the above, we have
\[
\Expect[Y] \geq (\vol(S)/2) \Prob[Y < (1/2)\vol(S)] + 4 \vol(S) (1 - \Prob[Y < (1/2)\vol(S)]) \geq  2 \vol(S),
\]
and this implies $\Prob[Y < (1/2)\vol(S)] \leq 4/7$.
We argue that $Y \geq (1/2)\vol(S)$ implies that either Condition~\ref{XXX-P3a} or Condition~\ref{XXX-P3b} holds. If Case~1 ever occurs, then the algorithm terminates before the last iteration $i=s$, and so we must have $\vol(C) \geq (1/48)\vol(V)$.
Similarly, if Case~2 ever occurs, we automatically have $\vol(C) \geq (1/48)\vol(V)$. Now assume Case~1 and Case~2 never occurs for all $j \in [1,h]$, then we have $\vol(C \cap S) \geq Y > (1/2)\vol(S)$.

We divide all $s$ iterations into $\ceil{\log_{7/4}(1/p)}$ intervals of length $h = 4g(\phi, \vol(V))$, and apply the above analysis to each of them. We conclude that with probability at least $1 - (4/7)^{\ceil{\log_{7/4}(1/p)}} \geq 1 - p$, there is at least one interval satisfying $Y \geq (1/2) \vol(S)$. In other words,   with probability at least $1 - p$, either Condition~\ref{XXX-P3a} or Condition~\ref{XXX-P3b} holds.
\end{proof}

\subsection{Distributed Implementation\label{XXX-sect-partition-impl}}

In this section we show that 
the algorithm \balancedcut($G, \phi$) can be implemented to run in $O(D \cdot \poly(\log n, 1/\phi))$ rounds in $\CONGEST$. We do not make effort in optimizing the round complexity.

\paragraph{Notations.} We often need to run our algorithms on a subgraph $G=(V,E)$ of the underlying communication network $G^\ast$, and so $|V|$ might be much smaller than the number of vertices $n$ in the actual communication network $G^\ast$. 
Nonetheless, we  still express the round complexity in terms of $n$. The parameter $n$ also indicates that the maximum allowed failure probability is $1 - 1/\poly(n)$.

In the implementation we sometimes need to broadcast certain information to the entire subgraph $G=(V,E)$ under consideration. Thus, the round complexity might depend on the parameter $D$, which is the diameter of $G$. However, in some scenario $G$ might be a subgraph of some other graph $G'$, and all edges within $G'$ can also be used for communication.
If the diameter of $G$ is much larger than the diameter of $G'$, then it is more efficient to do the broadcasting using the edges outside of $G$. In such a case, we can set $D$ as the diameter of $G'$, and our analysis still applies.

\begin{lemma}[Implementation of \distnibble]\label{XXX-lem-dist-nibble-impl}
Suppose $v$ initially knows that it is the starting vertex.
The algorithm  \distnibble$(G,v,\phi,b)$ can be implemented to run in $O\left(\frac{\log^6 n}{\phi^5}\right)$ rounds. Only the edges in $P^\ast$ participate in the computation. By the end of the algorithm, each vertex $u$ knows whether or not $u \in C$ w.h.p.
\end{lemma}
\begin{proof}
The proof is similar to the distributed implementation described in~\cite[Section 3.2]{ChangPZ19}.
First of all, the calculation of $q_t(u)$ and $r_t(u)$  for each $0 \leq t \leq \tlast$ for each vertex $u \in V$ can be done in $\tlast = O\left(\frac{\log^2 n}{\phi^2}\right)$ rounds.

Next, we have to go over all $O\left(\frac{\log n}{\phi}\right)$ choices of $x$ and all $ O\left(\frac{\log^2 n}{\phi^2}\right)$ choices of $t$ to see if there is a pair $(t,j)$ meeting the required four conditions. More specifically, given $t$ and $x$, our task is the following.

\paragraph{Search for $j$ and $S_j(q_t)$.}
We need to compute the index $j$ that is the smallest index satisfying $\vol(S_j(q_t)) \geq (1+\phi)^x$, and then compute the set $S_j(q_t)$. We show that this can be done in  $O(\tlast \log n) =  O\left(\frac{\log^3 n}{\phi^2}\right)$ rounds via a ``random binary search'' on the vertex set  $U$ containing all vertices $u$ with $q_t(u) > 0$. 
For the sake of presentation, we rank all vertices $u_1, \ldots, u_{|U|}$ by decreasing order of $q_t(u) / \deg(u)$. Note that each $u_i$ does not know its rank $i$, and we cannot afford to compute the rank of all vertices in $U$. Also note that $S_i(q_t) = \{u_1, \ldots, u_i\}$.


We maintain two indices $L$ and $R$ that control the search space. Initially, $L \gets 1$ and $R \gets |U|$. In each iteration, we  pick one vertex $u_i$ from $\{u_L, \ldots, u_R\}$ uniformly at random, and calculate $\vol(S_i(q_t))$. This can be done in $O(\tlast)$ rounds. More specifically, we build a spanning tree $T$ of the edge set $P^\ast$ rooted at $v$, and use the tree for communication. It is clear that the subgraph induced by $P^\ast$ is connected and has diameter $O(\tlast)$.


If $\vol(S_i(q_t)) < (1+\phi)^x$, we update $L \gets i$; if $\vol(S_i(q_t)) = (1+\phi)^x$, we update $L \gets i$ and $R \gets i$; otherwise we update  $R \gets i-1$.  We are done when we reach $L = R$.

In each iteration, with probability $1/2$ the rank of the vertex we sample lies in the middle half of $[L,R]$,  and  so the size of search space 
$[L,R]$ is reduced by a factor of at least $3/4$. 
Thus, within $O(\log n)$ iterations we have $L = R$, and $S_j(q_t) = \{u_1, \ldots, u_j\}$ with  $j = L = R$.
%Therefore, w.h.p., 
%after $O(\log n)$ iterations, we will have isolated $L = R = %j$. Thus, 
The round complexity of this procedure is $O(\tlast \log n) =  O\left(\frac{\log^3 n}{\phi^2}\right)$.

\paragraph{Checking  (C.1*), (C.2*), and (C.3).} Given the index $j$ and the subset $S_j(q_t)$, it is straightforward to check these three conditions in $O(\tlast)$ rounds.

\paragraph{Checking  (C.4).}
We first note that this condition does not depend on $j$, and so we only need to do this test once for each $t$. Testing this condition can also be done via a random binary search, as described above, and this takes also $O(\tlast \log n) =  O\left(\frac{\log^3 n}{\phi^2}\right)$ rounds.


\paragraph{Round Complexity.} To summarize,  we go over all $O\left(\frac{\log n}{\phi}\right)$ choices of $x$ and all $ O\left(\frac{\log^2 n}{\phi^2}\right)$ choices of $t$, and for each pair $(t,x)$ we have to spend $O\left(\frac{\log^3 n}{\phi^2}\right)$ rounds. Therefore, the total round complexity is $O\left(\frac{\log^6 n}{\phi^5}\right)$.
\end{proof}

\begin{lemma}[Implementation of \balancedcut]\label{XXX-lem-parallel-nibble-impl}
The algorithm \parallelnibble$(G, \phi)$ can be implemented to run in $O\left(D \log n + \frac{\log^7 n}{\phi^5}\right)$ rounds in $\CONGEST$.
\end{lemma}
\begin{proof}
The implementation of \parallelnibble($G, \phi$) has three parts. 

\paragraph{Generation of \distnibble\ Instances.}
The first part is to generate all $k$ instances of \distnibble($G,v,\phi,b$), where the starting vertex $v \sim \psi_V$ is sampled according to the degree distribution, and $b \in [1, \ell]$ is sampled with $\Prob[b = i] = 2^{-i} / (1 - 2^{-\ell})$.

Following the idea of~\cite[Lemma 3.6]{ChangPZ19}, this task can be solved in $O(D + \log n)$ rounds, as follows. 
We build a BFS tree rooted at an arbitrary vertex $x$. For each vertex $v$, define $s(v)$ as the sum of $\deg(u)$ for each $u$ in the subtree rooted at $v$. In $O(D)$ rounds we can let each vertex $v$ learn the number $s(v)$ by a bottom-up traversal of the BFS tree. 

We let the root vertex $x$ sample the parameter $b$ for all $k$ instances of \distnibble.
Denote $K_i$ as the number of instances with $b = i$.
At the beginning, the root $x$ stores $K_i$ amount of $i$-tokens.
Let $L=\Theta(D)$ be the number of layers in the BFS tree. For $j = 1, \ldots, L$, the vertices of layer $j$ do the following. When an $i$-token arrives at $v$, 
the $i$-token disappears at $v$ with probability $\deg(v)/s(v)$
and $v$ locally generates an instance of \distnibble\ with starting vertex $v$ and parameter $b = i$;
otherwise, $v$ passes the $i$-token to a child $u$ 
with probability $\frac{s(u)}{s(v)-\deg(v)}$. Though $v$ might need to send a large amount of $i$-tokens to $u$, the only information $v$ needs to let $u$ know it the number of $i$-tokens.
%Note that $v$ only needs to tell each child $u$ 
%how many $i$-tokens $u$ gets.  
Thus, for each $i$, the generation of all $K_i$ instances of \distnibble\ with a random starting vertex can be done in 
$L$ rounds. Using pipelining, we can do this for all $i$ in $O(D+\log n)$ rounds, independent of $k$.

\paragraph{Simultaneous Execution of \distnibble.} The second part is to run all $k$ instances of \distnibble\ simultaneously. If there is an edge $e$ participating in more than $w = O(\log n)$ of them, then the two endpoints of $e$ broadcast a special message $\star$ to everyone else to notify them to terminate the algorithm with $C = \emptyset$, and the broadcasting takes $D$ rounds. Otherwise, this task can be done in $O(\log n) \cdot O\left(\frac{\log^6 n}{\phi^5}\right) = O\left(\frac{\log^7 n}{\phi^5}\right)$ rounds in view of Lemma~\ref{XXX-lem-dist-nibble-impl}. Overall, the round complexity is $O\left(D + \frac{\log^7 n}{\phi^5}\right)$.


\paragraph{Selection of $i^\ast$ and $C = U_{i^\ast}$.} In the description of the algorithm \parallelnibble($G, \phi$), we assume that all \distnibble\ instances are indexed from $1$ to $k$. However, in a distributed implementation we cannot afford to do this. What we can do is to let the starting vertex $v$ of each \distnibble\ instance locally generate a random $O(\log n)$-bit identifier associated with the \distnibble\ instance. We say that an \distnibble\ instance is the $i$th instance if its identifier is ranked $i$th in the increasing order of all $k$ identifiers. 
With these identifiers, we can now use a random binary search to find $i^\ast$ and calculate $C = U_{i^\ast}$ in $O(D \log n)$ rounds w.h.p.

\paragraph{Round Complexity.} To summarize, the round complexity for the three parts are $O(D+\log n)$, $O\left(D + \frac{\log^7 n}{\phi^5}\right)$, and $O(D \log n)$. Thus, the total round complexity is $O\left(D \log n + \frac{\log^7 n}{\phi^5}\right)$.
\end{proof}



\begin{lemma}[Implementation of \balancedcut]\label{XXX-lem-partition-nibble-impl}
The algorithm \balancedcut$(G, \phi, p)$ with $p = 1/\poly(n)$ can be implemented to run in $O\left(\frac{D \log^9 n}{\phi^4}+ \frac{\log^{15} n}{\phi^{9}}\right)$ rounds in $\CONGEST$.
\end{lemma}
\begin{proof}
This lemma follows immediately from Lemma~\ref{XXX-lem-parallel-nibble-impl}, as \balancedcut($G, \phi$) consists of 
\[s = O\left(g(\phi, \vol(V)) \log(1/p)\right)  = O\left(\frac{\log^8 n}{\phi^4}\right)\] iterations of \parallelnibble, where each of them costs $O\left(D \log n + \frac{\log^7 n}{\phi^5}\right)$ rounds, and so the total round complexity is  $O\left(\frac{D \log^9 n}{\phi^4}+ \frac{\log^{15} n}{\phi^{9}}\right)$.
\end{proof}


==> Backup/sss.tex <==
\section{Nearly Most Balanced Sparse Cut} \label{XXX-sect-balanced-cut}
   
The goal of this section is to prove the following theorem.




\restatenearlybalcut*
\begin{proof}
This theorem follows from a re-parameterization of Lemma~\ref{XXX-lem-partition-nibble} and  Lemma~\ref{XXX-lem-partition-nibble-impl}.
\end{proof}



Given a parameter $\phi \in (0,1)$, We define the following functions as in~\cite{SpielmanT13}, where the values of the constants are $c_1 = 200$, $x_2 = 280$, $c_3 = 1800$, and $c_4 = 140$. The constant $c_4$ is used in the definition of \nibble.
\begin{align*}
    \ell &\bydef \ceil{\log(\vol(V))},\\
    \tlast &\bydef (\ell+1)\ceil{(2/\phi^2) \ln\left( c_1 (\ell+2) \sqrt{\vol(V) / 2}\right)},\\
    f_1(\phi) &\bydef \frac{1}{c_2(\ell+2) \tlast},\\
    \epsilon_b &\bydef 1/\left(c_3 (\ell+2) \tlast 2^b\right).
\end{align*}

Let $A$ be the adjacency matrix of the graph $G=(V,E)$.
We assume a 1-1 correspondence between $V$ and $\{1, \ldots, n\}$.
In a \textit{lazy random walk}, the walk stays at the current vertex with probability $1/2$ and otherwise moves to a random neighbor of the current vertex.
The matrix realizing this walk can be expressed as
 $M = (A D^{-1} + I) / 2$,
  where $D$ is the diagonal matrix with
  $(\deg(1), \ldots , \deg(n))$ on the diagonal.
  
Let $p_t^v$ be the probability distribution of the lazy random walk that begins at $v$ and walks for $t$ steps.
In the limit, as $t\rightarrow \infty$, 
$p_t(x)$ approaches $\deg(x)/2m$, so it is natural to measure 
$p_t(x)$ \emph{relative} to this baseline.
\[
\rho_t(x)=p_t(x)/\deg(x),
\]
%Define $\pi_t$ to be the permutation that sorts $V=\{1,\ldots,n\}$ in decreasing order of $\rho_t$-values, breaking ties by vertex ID. 

Let $p:  V \mapsto [0,1]$ be any function. 
The truncation operation $[p]_\epsilon$ 
rounds $p(x)$ to zero if it falls below a threshold that depends on $x$.
\[
  [p]_{\epsilon} (x)
=
\begin{cases}
  p (x) & \text{if $p (x) \geq \epsilon \deg(x)$,}\\
  0 & \text{otherwise}.
\end{cases}
\]
For each $1 \leq j \leq |V|$, we write $S_j(p)$ to denote the set of the top $j$ vertices with the highest $p(v)/\deg(v)$-value, breaking ties by comparing IDs. We also write $\lambda_j(p) = \vol(S_j)$.


As in~\cite{SpielmanT13}, for any vertex set $S$, we define the vector  $\chi_S$ by $\chi_S(u) = 1$ if $u \in S$ and $\chi_S(u) = 0$ if $u \notin S$, and we define the vector  $\psi_S$ by $\psi_S(u) = \deg(u) / \vol(S)$ if $u \in S$ and $\psi_S(u) = 0$ if $u \notin S$. In particular, $\chi_v$ is a probability distribution on $V$ that has all its probability mass on the vertex $v$, and $\psi_V$ is the degree distribution of $V$. 

\subsection{Nibble}
We first review the \nibble\ algorithm of~\cite{SpielmanT13}, which computes the following two sequences of vectors with truncation parameter $\epsilon_b$.
\begin{align*}
q_t &=\begin{cases}
\chi_v & \text{if $t = 0$,}\\
M r_{t-1} & \text{otherwise.}
\end{cases}\\
r_t & = [q_t]_{\epsilon_b}.
\end{align*}
We note that the following is true for all $u \in V$ and $t \geq 0$.
\[p_t(u) \geq q_t(u) \geq r_t(u).\]


\begin{framed}
\noindent {\bf Algorithm} \nibble($G,v,\phi,b$)

\medskip

For $t  = 1$ to $\tlast$, if there exists an index $1 \leq j \leq |V|$ meeting the following four conditions 
\begin{enumerate}
\addtolength{\itemindent}{1cm}
    \item[(C.1)] $\Phi(S_j(q_t)) \leq \phi$.
    \item[(C.2)] $\lambda_j(q_t) \leq (5/6) \vol(V)$.
    \item[(C.3)] $2^b \leq \lambda_j(q_t)$. 
    \item[(C.4)] Let $j^\ast$ be the smallest index such that $2^b \leq \lambda_{j^\ast}(q_t)$. Then $q_t(u) / \deg(u) \geq \frac{1}{c_4 (\ell+2) 2^b}$ for each  $u \in S_{j^\ast}(q_t)$.
\end{enumerate}
then return $C = S_j(q_t)$ and quit.
Otherwise return $C = \emptyset$.
\end{framed}

Note that the definition of \nibble($G,v,\phi,b$) is exactly the same as the one presented in~\cite{SpielmanT13}. In~\cite{SpielmanT13}, (C.4) is written alternatively and equivalently as $I_x(q_t, 2^b) \geq \frac{1}{c_4 (\ell+2) 2^b}$. 


\begin{definition}
 Define $Z_{u,\phi,b}$ as the subset of $V$ such that if we start the lazy random walk from $v \in Z_{u,\phi,b}$, then $\rho_t(u) \geq \epsilon_b$ for at least one of  $t \in [0, \tlast]$. 
 For any edge $e = \{u_1, u_2\}$, define $Z_{u,\phi,e} = Z_{u_1,\phi,b} \cup Z_{u_2,\phi,b}$.
 \end{definition}
 
 Intuitively, if $v \notin Z_{u,\phi,e}$, then $e$ does not  participate in \nibble($G,v,\phi,b$). Note that $v \in Z_{u,\phi,e}$ is  a necessary but not sufficient condition for $e \in E(C)$, where $C$ is the output of \nibble($G,v,\phi,b$).
The following auxiliary lemma establishes upper bounds on $\vol(Z_{u,\phi,b})$ and $\vol(Z_{e,\phi,b})$. This lemma will be applied to bound the amount of congestion when we execute multiple \nibble\ in parallel. Intuitively, if $\vol(Z_{e,\phi,b})$ is small, then we can afford to run many instances \nibble($G,v,\phi,b$) in parallel for random starting vertices $v$ sampled from the degree distribution $\psi_V$.

\begin{lemma}\label{XXX-lem-nibble-aux}
The following formulas hold for each vertex $u$ and each edge $e$.
\begin{align*}
    &\vol(Z_{u,\phi,b}) \leq (\tlast+1) / \epsilon_b\\
    &\vol(Z_{e,\phi,b}) \leq 2(\tlast+1) / \epsilon_b
\end{align*}
In particular, these two quantities are both upper bounded by $3 c_3 \tlast^2 \ell 2^b = O\left(\frac{ 2^b  \log^5 \vol(V)}{\phi^4}\right)$.
\end{lemma}
\begin{proof}
In this proof we use superscript to indicate the starting vertex of the lazy random walk.
We write $Z_{u,\phi,b,t} = \{ v \in V \ | \ \rho_t^v(u) \geq \epsilon_b \}$. Then $\vol(Z_{u,\phi,b}) \leq \sum_{t = 0}^{\tlast} \vol(Z_{u,\phi,b,t})$. Thus, to prove the lemma, if suffices to show that $\vol(Z_{u,\phi,b,t}) \leq 1 / \epsilon_b$.
This inequality follows from the fact that $\rho_t^v(u) = \rho_t^u(v)$, as follows.
\begin{align*}
1 &= \sum_{v \in V} p_t^u(v) \\
&\geq  \sum_{v \in V \ | \ \rho_t^u(v) \geq \epsilon_b} p_t^u(v) \\
&\geq \sum_{v \in V \ | \ \rho_t^u(v) \geq \epsilon_b} \epsilon_b \cdot \deg(v) \\
&= \sum_{v \in V \ | \ \rho_t^v(u) \geq \epsilon_b} \epsilon_b \cdot \deg(v) \\
&= \epsilon_b \cdot  \vol(Z_{u,\phi,b,t}).
\end{align*}
The fact that $\rho_t^v(u) = \rho_t^u(v)$ as been observed in~\cite{SpielmanT13} without a proof. 
For the sake of completeness, we will show a proof of this fact. An alternate proof can be found in~\cite[Lemma 3.7]{ChangPZ19}. In the following calculation, we use the fact that $D^{-1} M D = D^{-1}(AD^{-1}+I)D/2 = (D^{-1}A + I)/2 =  M^{\top}$.
\begin{align*}
    \rho_t^v(u) &= \chi_u^\top D^{-1} M^t \chi_v\\
    &= \chi_u^\top (D^{-1} M D)^t   (D^{-1}\chi_v)\\
    &= \chi_u^\top (M^{\top})^t   (D^{-1}\chi_v)\\
    &=  (D^{-1}\chi_v)^\top M^t \chi_u \\
    &=  \chi_v^\top D^{-1}  M^t \chi_u \\
    &= \rho_t^u(v).
\end{align*}
Finally, recall that $\epsilon_b = 1/\left(c_3 (\ell+2) \tlast 2^b\right)$, and so 
$2(\tlast + 1)/\epsilon_b =  2(\tlast + 1) \cdot c_3 (\ell+2) \tlast 2^b <  3 c_3 \tlast^2 \ell 2^b$. We assume that $\vol(V)$ is at least a sufficiently large constant so that the above calculation holds.
\end{proof}

 Lemma~\ref{XXX-lem-nibble} lists some crucial properties of \nibble.   In subsequent discussion, for any given subset $S\subset V$, the subset $S^g \subseteq S$ and the partition $S^g = \bigcup_{b=1}^{\ell} S^g_b$  are defined according to Lemma~\ref{XXX-lem-nibble}. 
 

\begin{lemma}[Analysis of \nibble]\label{XXX-lem-nibble}
For each $\phi \in (0,1]$, and for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi),
\end{align*}
there exists a subset $S^g \subseteq S$ with the following properties.
First, $\vol(S^g)\geq \vol(S)/2$.  Second, $S^g$ is partitioned into
$S^g = \bigcup_{b=1}^{\ell} S^g_b$ such that if a lazy random walk is initiated
at any $v\in S^g_b$ with truncation parameter
$\epsilon_b$, the following is true.
\begin{enumerate}
    \item\label{XXX-N1} The set $C$ returned by \nibble$(G,v,\phi,b)$ is non-empty.
    \item\label{XXX-N2} 
    Let $1 \leq t \leq  \tlast$, and let $j^\ast$ be the smallest index such that $2^b \leq \lambda_{j^\ast}(q_t)$. If    $q_t(u) / \deg(u) \geq \frac{1}{c_4 (\ell+2) 2^b}$ for each  $u \in S_{j^\ast}(q_t)$, then  $\vol(S_{j^\ast}(q_t) \cap S) \geq 2^{b-1}$.
\end{enumerate}
\end{lemma}
\begin{proof}
The first condition follows from~\cite[Theorem 2.1 (N.3)]{SpielmanT13}. The second condition follows from the proof of~\cite[Lemma 2.8]{SpielmanT13}. 
\end{proof}

To put it another way, Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N1}) says that there exist  $1 \leq t \leq  \tlast$ and $1 \leq j \leq |V|$ such that (C.1)--(C.4) are met;   Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N2}) says that for any choice of  $1 \leq t \leq  \tlast$   satisfying (C.4), we have $\vol(S_{j^\ast}(q_t) \cap S) \geq 2^{b-1}$, where $j^\ast$ is the index considered in (C.4).

Intuitively, the set $S^g$ represents the ``core'' of $S$ in the sense that \nibble$(G,v,\phi,b)$  is guaranteed to return a  sparse cut $C$ if $v \in S_b^g$. Recall that (C.1) and (C.2) in the description of \nibble$(G,v,\phi,b)$ guarantees that the cut $C$ has conductance at most $\phi$ and has volume at most $(5/6)\vol(V)$.

\subsection{Approximate Nibble}
The  algorithm \nibble\ is not suitable for a distributed implementation since it has to go over all possible $j$. Similar to the idea of~\cite[Algorithm~1]{ChangPZ19} we provide a slightly modified version of \nibble\ that only considers $O((1/\phi)\log n)$ choices of $j$ for each $t$.
The cost of doing so is that we have to relax the two conditions (C.1) and (C.2) slightly.

\begin{framed}
\noindent {\bf Algorithm} \distnibble($G,v,\phi,b$)

\medskip

For $t  = 1$ to $\tlast$, and for $x = 0$ to $\floor{\log_{1+\phi} (5/6)\vol(V)}$, set  $j$ as the smallest index such that $\vol(S_j(q_t)) \geq (1+\phi)^x$. If the parameter $j$ meets the following four conditions
\begin{enumerate}
\addtolength{\itemindent}{1cm}
    \item[(C.1*)] $\Phi(S_j(q_t)) \leq 12\phi$.
    \item[(C.2*)] $\lambda_j(q_t) \leq (11/12) \vol(V)$.
    \item[(C.3)] $2^b \leq \lambda_j(q_t)$.
    \item[(C.4)] Let $j^\ast$ be the smallest index such that $2^b \leq \lambda_{j^\ast}(q_t)$. Then $q_t(u) / \deg(u) \geq \frac{1}{c_4 (\ell+2) 2^b}$ for each  $u \in S_{j^\ast}(q_t)$.
\end{enumerate}
then return $C = S_j(q_t)$ and quit.
Otherwise return $C = \emptyset$.
\end{framed}



\begin{definition}
Consider \distnibble$(G,v,\phi,b)$. Define $P^\ast$ as the set of edges  $e$ such that there exist at least one endpoint $u$ of $e$ and at least one number $t \in [0, \tlast - 1]$ with $r_t(u) > 0$.
\end{definition}

 Intuitively,   $P^\ast$  is the set of edges that participate in   \distnibble($G,v,\phi,b$). This notation will be used in analyzing the complexity of our distributed implementation.


\begin{definition}
Consider \distnibble$(G,v,\phi,b)$. 
If the output $C$ is non-empty, then define $C^\ast = \{ u \in C \ | \ \rho_t(u) \geq \epsilon_b \}$, where $t$ is the index such that $C = S_j(q_t)$; otherwise define  $C^\ast = \emptyset$.
\end{definition}

Due to the facts that $\epsilon_b < \frac{1}{c_4 (\ell+2) 2^b}$ and $\rho_t(u) = p_t(u)/\deg(u) \geq q_t(u)/\deg(u)$, we always have $S_{j^\ast}(q_t) \subseteq C^\ast$, where $j^\ast$ is the index considered in (C.4), for the case the output $C$ is non-empty.

Regardless of the choice of $b$ and $v$, the output $C$ of \distnibble$(G,v,\phi,b)$ must satisfy $\Phi(C) \leq 12\phi$ and   $\vol(C) \leq (11/12) \vol(V)$. Lemma~\ref{XXX-lem-dist-nibble} shows an additional property of $C$ when $v$ is appropriately chosen.

\begin{lemma}[Analysis of \distnibble]\label{XXX-lem-dist-nibble}
For each $0 < \phi \leq 1/12$, and for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi),
\end{align*}
the output $C$ of \distnibble$(G,v,\phi,b)$ for any $v \in S_g^b$ satisfies 
\[\vol(C \cap S) \geq \vol(C^\ast \cap S)  \geq 2^{b-1}.\]
\end{lemma}
\begin{proof}
We pick $(t,j)$ as the indices that satisfy (C.1)--(C.4), whose existence is guaranteed by Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N1}). Let $v \in S_g^b$. We first show that the output $C$ of \distnibble$(G,v,\phi,b)$ is non-empty. That is, we argue that there exists an index $j' \geq j$ such that the pair  $(t,j')$ is under consideration in \distnibble($G,v,\phi,b$) and it satisfies all four conditions (C.1*), (C.2*), (C.3), and (C.4). 
Remember that an index $j'$ is under consideration in 
\distnibble($G,v,\phi,b$) if there exists an integer $x$ within the range $[0, \log_{1+\phi} (5/6)\vol(V)]$ such that $j'$ is the smallest index satisfying  $\vol(S_{j'}(q_t)) \geq (1+\phi)^x$. More specifically, we select $j'$  as the smallest index such that $j' \geq j$ and $j'$ is considered in \distnibble($G,v,\phi,b$).
Since $t$ is fixed, from now on we write $S_j$ as a shorthand for  $S_j(q_t)$, and $S_{j'}$ for $S_{j'}(q_t)$.  


\paragraph{Conditions (C.1*) and (C.2*).} We first verify that (C.1*) and (C.2*) are met. We divide the analysis into two cases.
\begin{itemize}
\item Consider the case $\vol(S_{j'}) \leq \vol(V)/2$. We have $|\partial(S_{j'})| \leq |\partial(S_j)| + \phi \vol(S_j) \leq 2\phi \vol(S_j) \leq 2\phi \vol(S_{j'})$, and so $\Phi(S_{j'}) = |\partial(S_{j'})| / \vol(S_{j'}) \leq 2\phi$, and so (C.1*) is met.
In the above calculation, we use the fact that $|\partial(S_j)| \leq \phi \vol(S_j)$, which is due to the assumption that  $(t,j)$ satisfies (C.1).
Note that (C.2*) is automatically met in this case.


\item Consider the case $\vol(S_{j'}) > \vol(V)/2$.
The following calculation shows that (C.2*) is met. The calculation uses the facts that $\phi \leq 1/12$ and $\vol(V \setminus S_{j}) \geq (1/6)\vol(V)$, where the latter is due to the assumption that  $(t,j)$ satisfies (C.2).
\begin{align*}
    \vol(V \setminus S_{j'}) &\geq
    \vol(V \setminus S_{j}) - \phi \vol(S_j) \\
    &\geq \vol(V \setminus S_{j}) - (1/12)\vol(S_j)\\
    &\geq \vol(V \setminus S_{j}) - (1/12)\vol(V)\\
    &\geq \vol(V \setminus S_{j}) / 2\\
    &\geq (1/12)\vol(V).
\end{align*}
Similarly, we have $|\partial(S_j')| \leq \phi \vol(V \setminus S_{j}) + \phi \vol(S_j)$. 
Since $\vol(S_{j}) \leq (5/6)\vol(V)$, we have $\phi \vol(S_j) \leq 5 \phi \vol(V \setminus S_j)$.
Therefore, $|\partial(S_j')| \leq 6\phi \vol(V \setminus S_{j}) \leq 12\phi  \vol(V \setminus S_{j'})$, which implies  (C.1*).
\end{itemize}


\paragraph{Conditions (C.3)  and (C.4).}
We also observe that (C.3)  and (C.4) also hold for the parameters $(t,j')$, as follows. Remember that (C.3)  and (C.4) hold for the parameters $(t,j)$. Since $\lambda_{j'}(q_t) > \lambda_{j}(q_t)$ so long as $j' > j$, we infer that (C.3) also holds for  $(t,j')$.  Also,  (C.4) automatically holds for  $(t,j')$ since this condition only depends on $t$.


\paragraph{Lower Bound of $\vol(C^\ast \cap S)$.}
Finally, we prove that $\vol(C^\ast \cap S) \geq 2^{b-1}$.
Select $j^\ast$ as the index considered in (C.4). Note that we must have $j^\ast \leq j \leq j'$.
By definition of $C^\ast$, we have $S_{j^\ast} \subseteq C^\ast \subseteq S_{j'} = C$.  Therefore, all we need to do is to show that $\vol(S_{j^\ast} \cap S) \geq 2^{b-1}$.
This follows from Lemma~\ref{XXX-lem-nibble}(\ref{XXX-N2}) and the fact that $t$ satisfies (C.4).
\end{proof}

Lemma~\ref{XXX-lem-dist-nibble} implicitly shows that if $v \in S_g^b$, then the output $C$ of \distnibble$(G,v,\phi,b)$ is non-empty, and so it has conductance at most $12 \phi$ and volume at most $(11/12)\vol(V)$ in view of (C.1*) and (C.2*). 

Recall that the main goal of Section~\ref{XXX-sect-balanced-cut} is to design a distributed algorithm that finds a nearly most balanced sparse cut, so finding a cut $C$ satisfying (C.1*) and (C.2*) is not enough. This is in contrast to~\cite{ChangPZ19}, where they do not need the output cut to satisfy any balance constraint.

Following the approach of~\cite{SpielmanT13}, to find a nearly most balanced sparse cut, we will need to take the union of the output of multiple instances of \distnibble, and the goal of the analysis is to show that the resulting vertex set has volume at least $\vol(S)/2$.  
This explains the reason why we not only need to show that $C \neq \emptyset$ but also  need to show a lower bound of $\vol(C \cap S)$ in Lemma~\ref{XXX-lem-dist-nibble}.





\subsection{Random Nibble}
Note that both \nibble\ and \distnibble\ are deterministic. Next, we consider the algorithm \randnibble\ which executes \distnibble\ with a random starting vertex $v$ and a random parameter $b$. The definition of  \randnibble\ exactly the same as the corresponding one in~\cite{SpielmanT13} except that we use \distnibble\ instead of \nibble.


\begin{framed}
\noindent {\bf Algorithm} \randnibble($G,\phi$)

\medskip

Sample a starting vertex $v \sim \psi_V$ according to the degree distribution. Choose a number $b \in [1, \ell]$ with $\Prob[b = i] = 2^{-i} / (1 - 2^{-\ell})$. Execute \distnibble($G,v,\phi,b$), and return the result $C$.
\end{framed}

Note that the set of edges $P^\ast$ participating in the subroutine \distnibble($G,v,\phi,b$) satisfies that $P^\ast \subseteq E(C)$, where $C$ is the output of  \randnibble($G,\phi$). Therefore, Lemma~\ref{XXX-lem-rand-nibble} also implies that  $\Prob[e \in E(C)] \leq (4 c_3 \tlast^2 \ell^2) /\vol(V)$ for each $e \in E$.



\begin{lemma}[Analysis of \randnibble]\label{XXX-lem-rand-nibble}
For each $0 < \phi \leq 1/12$, the following holds for the output $C$ of \distnibble$(G,v,\phi,b)$. 
\begin{enumerate}
    \item  $\Prob[e \in P^\ast] \leq (4 c_3 \tlast^2 \ell^2) /\vol(V)$ for each $e \in E$, where $P^\ast$ is the set of edges participating in the subroutine \distnibble$(G,v,\phi,b)$.
   % \item $\Prob[u \in C^\ast] \leq  (4 c_3 \tlast^2 \ell^2) /\vol(V)$ for each $u \in V$.
    \item  $\Expect[\vol(C \cap S)] \geq \Expect[\vol(C^\ast \cap S)] \geq \frac{\vol(S)}{4 \vol(V)}$ for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi).
\end{align*} 
\end{enumerate}
\end{lemma}
\begin{proof}
The proof of $\Expect[\vol(C^\ast \cap S)] \geq \frac{\vol(S)}{4 \vol(V)}$ follows from Lemma~\ref{XXX-lem-dist-nibble}  and the proof of~\cite[Lemma 3.1]{SpielmanT13}. An upper bound of $\Prob[e \in P^\ast]$ can be calculated using Lemma~\ref{XXX-lem-nibble-aux}. More specifically, observe that $v \in Z_{e,\phi,i}$ is a necessary condition for $e \in E(C)$ for the case $b = i$, and so we can upper bound $\Prob[e \in P^\ast]$ as follows.
\begin{align*}
    \Prob[e \in P^\ast] &\leq \sum_{i=1}^{\ell} \Prob[b = i] \cdot \vol(Z_{e,\phi,i}) / \vol(V)\\
    &\leq \sum_{i=1}^{\ell} \frac{2^{-i}}{1 - 2^{-\ell}} \cdot  (3 c_3 \tlast^2 \ell 2^i) /\vol(V)\\
    &< \sum_{i=1}^{\ell} (4 c_3 \tlast^2 \ell) /\vol(V)\\
    &=  (4 c_3 \tlast^2 \ell^2) /\vol(V). \qedhere
\end{align*}
%The calculation of $\Prob[u \in C^\ast]$ is similar, as we observe that $v \in Z_{u,\phi,i}$ is a necessary condition for $u \in C^\ast$ for the case $b = i$.
\end{proof}


%Lemma~\ref{XXX-lem-rand-nibble}(2) and Lemma~\ref{XXX-lem-rand-nibble}(3) will be crucial when we analyze the intersection of $S$ and the vertex set resulting from combining the output of multiple instances of \randnibble($G,\phi$).
%The proof of Lemma~\ref{XXX-lem-rand-nibble} explains the technical reason as to why we consider $C^\ast$ instead of $C$. The proof of the upper bound of $\Prob[u \in C^\ast]$ in  Lemma~\ref{XXX-lem-rand-nibble} does not hold if we replace $C^\ast$ with $C$. In principle, the set $C=S_j(q_t)$ might include vertices $u$ with very small $\rho_t(u)$-value. 
%For comparison, the analysis of~\cite{SpielmanT13} does not suffer from this issue since in their algorithm \randnibble($G,\phi$) is applied \emph{sequentially}, not  \emph{in parallel}. 


\subsection{Parallel Nibble} 
In~\cite{SpielmanT13}, roughly speaking, it was shown that a nearly most balanced sparse cut can be found with probability $1 - p$ by \emph{sequentially} applying \nibble\ with a random starting vertex for $O(|E| \log (1/p))$ times.
After each \nibble, the output subset $C$ is removed from the underlying graph. To achieve an efficient implementation in $\CONGEST$, we need to diverge from this approach and aim at doing multiple \distnibble\ \emph{in parallel}. 

However, the na\"{i}ve approach of doing all $O(|E| \log (1/p))$ \randnibble\ in parallel does not work, since the potentially high overlap between the output subsets of different execution of \randnibble\ will destroy the required conductance constraint.

In what follows, we consider the algorithm \parallelnibble, which involves a simultaneous execution of a moderate number of \distnibble.
In the description of \parallelnibble, we say that $e$ participates in the subroutine \randnibble($G,\phi$) if $e \in P^\ast$ for the subroutine \distnibble($G,v,\phi,b$) during the execution of \randnibble($G,\phi$).

\begin{framed}
\noindent {\bf Algorithm} \parallelnibble($G, \phi$)

\medskip

For $i = 1$ to $k \bydef \ceil{\vol(V) / (4 c_3 \tlast^2 \ell^2)}$, do \randnibble($G,\phi$), in parallel. Let $C_i$ be the result of the $i$th execution of \randnibble($G,\phi$). Let $U_i = \bigcup_{j=1}^i C_i$.  If there exists an edge $e$ participating in the subroutine \randnibble($G,\phi$) for more than $w \bydef 10 \ceil{\ln (\vol(V))}$ times, return $C = \emptyset$.
Otherwise select $i^\ast \in [1, k]$ to be the highest index such that $\vol(U_{i^\ast}) \leq z  \bydef (23/24)\vol(V)$. Return $C = U_{i^\ast}$.
\end{framed}

For the sake of presentation, in the statement of Lemma~\ref{XXX-lem-par-nibble} we define the function $g$ by
\[g(\phi, \vol(V)) \bydef 20 c_3 w \tlast^2  \ell^2.\]
In particular, we have $5w \vol(V)/k \leq g(\phi, \vol(V))$. The function $g$ will also be used in the description and the analysis of \balancedcut\ in the subsequent discussion. 
 
\begin{lemma}[Analysis of \parallelnibble]\label{XXX-lem-par-nibble}
For each $0 < \phi \leq 1/12$ 
the following is true for the output $C$ of \parallelnibble($G, \phi$).
\begin{enumerate}
    \item If $C \neq \emptyset$, then  $\Phi(C) \leq 276 w \phi$. 
    \item For each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{2}{3}\cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi),
\end{align*} define the random variable $y$ as follows.
\[
y = 
\begin{cases}
\vol(S), \text{ if } \vol(C) \geq (1/24)\vol(V) \\
\vol(C \cap S), \text{ otherwise}\\
\end{cases}
\]
Then $\Expect[y] \geq \frac{k \vol(S)}{5w \vol(V)} \geq \frac{\vol(S)}{g(\phi, \vol(V))}$.
\end{enumerate}
\end{lemma}
\begin{proof}
We show that if the output subset $C$ is non-empty, then we must have $\Phi(C) \leq 276 w \phi$. 
By definition of \parallelnibble, if the output is non-empty, then each edge $e$ is included in at most $w$ of these subsets $C_1, \ldots, C_{i^\ast}$. Therefore, $\vol(C) \geq (1/w) \sum_{i=1}^{i^\ast} \vol(C_i)$. 
We upper bound $|\partial(C)|$ as follows, where we use the fact that the output $C_i$ of \distnibble$(G,v,\phi,b)$ has $\Phi(C_i)\leq 12\phi$.
\begin{align*}
    |\partial(C)| &\leq \sum_{i=1}^{i^\ast} |\partial(C_i)|\\ &\leq  \sum_{i=1}^{i^\ast} 12 \phi \vol(C_i)\\
    &\leq 12 w \phi \vol(C).
\end{align*}
The threshold $z$ guarantees that $\vol(V \setminus C) \geq (1/23) \vol(C)$, and so $|\partial(C)|  \leq  12 \cdot 23 \cdot w \phi \vol(V \setminus C) = 276 w \phi \vol(V \setminus C)$. We conclude that $\Phi(C) \leq 276 w \phi$. 



Next, we analyze the random variable $y$. We first observe that if $i^\ast <  k$, then $C = U_{i^\ast}$ has $\vol(C) \geq (1/24) \vol(V)$.
This is because that each $C_i$ must have $\vol(C_i) \leq (11/12) \vol(V)$ by definition of \distnibble. 
If $\vol(U_{i^\ast}) < (1/24) \vol(V)$, then $\vol(U_{i^\ast + 1}) <   (1/24) \vol(V) +  (11/12) \vol(V) <  (23/24) \vol(V)$, contradicting the choice of $i^\ast$.
Thus, for the case $i^\ast <  k$, we automatically have $y = \vol(S)$, which is the maximum possible value of $y$. In view of this, we can lower bound $\Expect[y]$ as follows.
\[
\Expect[y] \geq \Expect[\vol(U_k \cap S)] - \Prob[B] \cdot \vol(S),
\]
where $B$ is the  event that there exists an edge  participating in the subroutine \randnibble($G,\phi$) for more than $w$ times.
Note that $B$ implies $C = \emptyset$, but not vise versa.

By Lemma~\ref{XXX-lem-rand-nibble}, we know that $\Expect[\vol(C_i \cap S)] \geq \frac{\vol(S)}{4 \vol(V)}$, and this implies $\Expect[\vol(U_k \cap S)] \geq (1/w) \sum_{i=1}^{k} \Expect[\vol(C_i)] = \frac{k\vol(S)}{4w \vol(V)}$.
Therefore, to obtain the desired bound $\Expect[y] \geq \frac{k\vol(S)}{5w \vol(V)}$, it remains to show that $\Prob[B] \leq \frac{k}{20w \vol(V)}$.


If $k = 1 \leq w$, then $\Prob[B] = 0$.
In what follows, we assume $k \geq 2$, and this implies
$k \leq 2 \cdot \vol(V) / (4 c_3 \tlast^2 \ell^2)$.
Let $e \in E$. Define $X_i = 1$ if $e$ participates in the $i$th \randnibble($G,\phi$), and define $X_i = 0$ otherwise. Set  $X = \sum_{i=1}^k X_i$.
By Lemma~\ref{XXX-lem-rand-nibble} and the inequality $k \leq 2 \cdot \vol(V) / (4 c_3 \tlast^2 \ell^2)$, we infer that $\Expect[X] \leq 2$. By a Chernoff bound, $\Prob[X > w] \leq \exp(- 2(w-2) / 3) \ll (\vol(V))^{-2}$. By a union bound over all edges $e \in E$, we infer that $\Prob[B] < (\vol(V))^{-1} \ll \frac{k}{20w \vol(V)}$, as required.
\end{proof}


Intuitively, Lemma~\ref{XXX-lem-par-nibble} shows that we only lose a factor of $O(\log n)$ in conductance if we combine the result of $k$ parallel executions of \randnibble($G,\phi$).
We are now ready to present the algorithm for finding a nearly most balanced sparse cut, which involves executing \parallelnibble\ sequentially for $s = O(\poly(1/\phi, \log n))$ times on the remaining subgraph.


\begin{framed}
\noindent {\bf Algorithm} \balancedcut($G, \phi, p$)

\medskip
 Initialize $W_0 = V$. For $i = 1$ to $s \bydef 4 g(\phi, \vol(V)) \ceil{\log_{7/4}(1/p)}$ do the following.
\begin{enumerate}
    \item Execute \parallelnibble($G\{W_{i-1}\}, \phi$). Let the output be $C_i$. 
    \item Set $W_i = W_{i-1} \setminus C_i$. 
    \item If $\vol(W_i) \leq (47/48)\vol(V)$ or $i=s$, return $C = \bigcup_{j=1}^i C_j$ and quit.
\end{enumerate}
\end{framed}


\begin{lemma}[Analysis of \balancedcut]\label{XXX-lem-partition-nibble}
Let $C$ be the output of \balancedcut($G, \phi$), with  $0 <  \phi \leq 1/12$.
Then the following holds:
\begin{enumerate}
\item \label{XXX-P1} $\vol(C) \leq (47/48) \vol(V)$.
\item \label{XXX-P2} If $C \neq \emptyset$, then $\Phi(C) =  O(\phi \log |V|)$.
\item \label{XXX-P3} Furthermore, 
for each subset $S\subset V$ satisfying
\begin{align*}
\vol(S) &\leq \frac{1}{2} \cdot \vol(V)
\text{ \ \ and \ \ \ } 
\Phi(S) \leq f_1(\phi) / 2,
\end{align*}
with probability at least $1-p$, at least one of the following holds:
\begin{enumerate}
    \item \label{XXX-P3a} $\vol(C) \geq (1/48)\vol(V)$.
    \item \label{XXX-P3b} $\vol(S \cap C) \geq (1/2) \vol(S)$.
\end{enumerate}
\end{enumerate}
\end{lemma}
\begin{proof} This proof follows the framework of~\cite[Theorem 3.2]{SpielmanT13}.

\paragraph{Proof of Condition~\ref{XXX-P1}.} 
Let $i'$ be the index such that the output subset $C$ is $\bigcup_{j=1}^{i'} C_j$. Then we have $\vol(C) \leq \vol(V \setminus W_{i'-1}) + \vol(C_{i'})$.
Since the algorithm does not terminate at the $(i'-1)$th iteration, we have $\vol(W_{i'-1}) > (47/48)\vol(V)$, and so
$\vol(V \setminus W_{i'-1}) \leq (1/48)\vol(V)$.
By the algorithm description of \parallelnibble, we have  $\vol(C_{i'}) \leq (23/24)\vol(W_{i'-1}) \leq (23/24)\vol(V)$. To summarize, we have $\vol(C) \leq (1/48)\vol(V) + (23/24)\vol(V) = (47/48)\vol(V)$.

\paragraph{Proof of Condition~\ref{XXX-P2}.} 
Note that the sets $C_1, \ldots, C_{i'}$ that constitute
 $C = \bigcup_{j=1}^{i'} C_j$ are disjoint vertex sets.
 We have $|\partial(C)| \leq \sum_{j=1}^{i'} |\partial(C_i)| \leq O(\phi \log |V|) \sum_{j=1}^{i'} \vol(C_i) =  O(\phi \log |V|) \cdot \vol(C)$, where the second inequality is due to Lemma~\ref{XXX-lem-par-nibble}.
 By Condition~\ref{XXX-P1}, we infer that $\vol(V \setminus C) \geq (1/48) \vol(C)$, and so we also have $|\partial(C)| \leq O(\phi \log |V|) \cdot \vol(V \setminus C)$. Hence $\Phi(C) = O(\phi \log |V|)$.


\paragraph{Proof of Condition~\ref{XXX-P3}.} 
 We focus on $h \bydef 4g(\phi, \vol(V))$ consecutive iterations from $i = x+1$ to  $i = x+h$, for some index $x$.
For each index $j \in [1, h]$, we write $H_j$ to denote  the event that (i) $\vol(S \cap W_{x+j-1}) \leq \vol(S)/2$ or (ii) the algorithm ends prior to iteration $i = x+j$. 
We define the random variable $Y_j$ as follows. 
\[
Y_j = 
\begin{cases}
\frac{\vol(S)}{2g(\phi, \vol(V))} &\text{ if $H_j$ occurs (Case 1)} \\
\vol(W_{x+j-1} \cap S) &\text{ if } \vol(C_{x+j}) \geq (1/24)\vol(W_{x+j-1}) \text{ (Case 2)} \\
\vol(C_{x+j} \cap S) &\text{ otherwise (Case 3)}\\
\end{cases}
\]
We  claim that if $H_j$ does not occur, then the preconditions of Lemma~\ref{XXX-lem-par-nibble} are  met for the cut $S' = S \cap W_{x+j-1}$ in the graph $G' = G\{ W_{x+j-1}\}$ when we run \parallelnibble($G\{W_{x+j-1}\}, \phi$) during the $(x+j)$th iteration.
\begin{itemize}
\item We show that $\vol(S \cap W_{x+j-1}) \leq (2/3) \vol(W_{x+j-1})$, as follows. 

\begin{align*}
  \vol(S \cap W_{x+j-1}) 
  &\leq (1/2) \vol(V)  &\vol(S) \leq \vol(V)/2\\
  &< (1/2)(48/47) \vol(W_{x+j-1}) &\vol(W_{x+j-1}) > (47/48) \vol(V)\\
  &< (2/3) \vol(W_{x+j-1}).
\end{align*}

\item We show that  $\Psi_{G\{ W_{x+j-1}\}}(S) \leq 2\Phi(S) \leq f_1(\phi, \vol(V)) \leq f_1(\phi, \vol(W_{x+j-1}))$, where we write $f_1(\phi, r)$ to indicate the value of $f_1(\phi)$ when the underlying graph has volume $r$.

\begin{align*}
  \Psi_{G\{ W_{x+j-1}\}}(S)
  &= \frac{|E(S\cap W_{x+j-1},  W_{x+j-1} \setminus S)|}{\min\{\vol(S\cap W_{x+j-1}),\vol(W_{x+j-1} \setminus S)\}}\\
  &\leq \frac{|E(S, V \setminus S)|}{\min\{\vol(S\cap W_{x+j-1}),\vol(W_{x+j-1} \setminus S)\}}\\
  &< \frac{|E(S, V \setminus S)|}{(1/2)\min\{\vol(S),\vol(V \setminus S)\}}\\
  &= 2\Phi(S).
\end{align*}
  
The second inequality is explained as follows.
We have $\vol(S \cap W_{x+j-1}) > \vol(S)/2$ since $H_j$ does not occur, and we also have

\begin{align*}
\vol(W_{x+j-1} \setminus S) &\geq \vol(V \setminus S) - (1/48)\vol(V)\\
&\geq \vol(V \setminus S) - (1/24)\vol(V \setminus S) &\vol(V \setminus S) \geq (1/2)\vol(V)\\
&> \vol(V \setminus S)/2.
\end{align*}
\end{itemize}
Thus, we are able to use Lemma~\ref{XXX-lem-par-nibble} to infer that   that \[\Expect[Y_j \ | \ \overline{H_j}] \geq \frac{\vol(S \cap W_{x+j-1})}{g(\phi, \vol(W_{x+j-1}))} > \frac{\vol(S)}{2g(\phi, \vol(V))}.\]
In the calculation we use the two inequalities $g(\phi, \vol(V)) \geq g(\phi, \vol(W_{x+j-1}))$ and $\vol(S \cap W_{x+j-1}) > \vol(S)/2$, where the latter is due to $\overline{H_j}$.
Combining $\Expect[Y_j \ | \ \overline{H_j}] > \frac{\vol(S)}{2g(\phi, \vol(V))}$ with the trivial bound  $\Expect[Y_j \ | \ {H_j}] =  \frac{\vol(S)}{2g(\phi, \vol(V))}$, we conclude that
 \[\Expect[Y_j] \geq \frac{\vol(S)}{2g(\phi, \vol(V))}.\] 
 
We write $Y = \sum_{j=1}^h Y_j$, and we have  $\Expect[Y] \geq 2 \vol(S)$ in view of the above, as we recall $h = 4g(\phi, \vol(V))$.
We claim that we always have $Y \leq 4\vol(S)$.
We may write $Y = Y^1 + Y^2 + Y^3$, where $Y^i$ considers the part of $Y$ due to Case~$i$ in the definition of $Y_j$. It is clear that $Y^1 \leq h \cdot \frac{\vol(S)}{2g(\phi, \vol(V))} = 2 \vol(S)$. We claim that  $Y^2 \leq \vol(S)$ by observing that Case~2 can only occur at most once.  Suppose Case~2  occurs at iteration $i = x+j$. Then $\vol(C_{x+j}) \geq
(1/24)\vol(W_{x+j-1}) > (1/48)\vol(W_{x+j-1})$, which implies $\vol(W_{x+j}) \leq (47/48)\vol(W_{x+j-1}) \leq  (47/48)\vol(V)$, and so the algorithm terminates.  For Case~3, we have $Y^3 \leq \sum_{j=1}^h \vol(C_{x+j} \cap S) \leq \vol(S)$.
In view of the above, we have
\[
\Expect[Y] \geq (\vol(S)/2) \Prob[Y < (1/2)\vol(S)] + 4 \vol(S) (1 - \Prob[Y < (1/2)\vol(S)]) \geq  2 \vol(S),
\]
and this implies $\Prob[Y < (1/2)\vol(S)] \leq 4/7$.
We argue that $Y \geq (1/2)\vol(S)$ implies that either Condition~\ref{XXX-P3a} or Condition~\ref{XXX-P3b} holds. If Case~1 ever occurs, then the algorithm terminates before the last iteration $i=s$, and so we must have $\vol(C) \geq (1/48)\vol(V)$.
Similarly, if Case~2 ever occurs, we automatically have $\vol(C) \geq (1/48)\vol(V)$. Now assume Case~1 and Case~2 never occurs for all $j \in [1,h]$, then we have $\vol(C \cap S) \geq Y > (1/2)\vol(S)$.

We divide all $s$ iterations into $\ceil{\log_{7/4}(1/p)}$ intervals of length $h = 4g(\phi, \vol(V))$, and apply the above analysis to each of them. We conclude that with probability at least $1 - (4/7)^{\ceil{\log_{7/4}(1/p)}} \geq 1 - p$, there is at least one interval satisfying $Y \geq (1/2) \vol(S)$. In other words,   with probability at least $1 - p$, either Condition~\ref{XXX-P3a} or Condition~\ref{XXX-P3b} holds.
\end{proof}

\subsection{Distributed Implementation\label{XXX-sect-partition-impl}}

In this section we show that 
the algorithm \balancedcut($G, \phi$) can be implemented to run in $O(D \cdot \poly(\log n, 1/\phi))$ rounds in $\CONGEST$. We do not make effort in optimizing the round complexity.

\paragraph{Notations.} We often need to run our algorithms on a subgraph $G=(V,E)$ of the underlying communication network $G^\ast$, and so $|V|$ might be much smaller than the number of vertices $n$ in the actual communication network $G^\ast$. 
Nonetheless, we  still express the round complexity in terms of $n$. The parameter $n$ also indicates that the maximum allowed failure probability is $1 - 1/\poly(n)$.

In the implementation we sometimes need to broadcast certain information to the entire subgraph $G=(V,E)$ under consideration. Thus, the round complexity might depend on the parameter $D$, which is the diameter of $G$. However, in some scenario $G$ might be a subgraph of some other graph $G'$, and all edges within $G'$ can also be used for communication.
If the diameter of $G$ is much larger than the diameter of $G'$, then it is more efficient to do the broadcasting using the edges outside of $G$. In such a case, we can set $D$ as the diameter of $G'$, and our analysis still applies.

\begin{lemma}[Implementation of \distnibble]\label{XXX-lem-dist-nibble-impl}
Suppose $v$ initially knows that it is the starting vertex.
The algorithm  \distnibble$(G,v,\phi,b)$ can be implemented to run in $O\left(\frac{\log^6 n}{\phi^5}\right)$ rounds. Only the edges in $P^\ast$ participate in the computation. By the end of the algorithm, each vertex $u$ knows whether or not $u \in C$ w.h.p.
\end{lemma}
\begin{proof}
The proof is similar to the distributed implementation described in~\cite[Section 3.2]{ChangPZ19}.
First of all, the calculation of $q_t(u)$ and $r_t(u)$  for each $0 \leq t \leq \tlast$ for each vertex $u \in V$ can be done in $\tlast = O\left(\frac{\log^2 n}{\phi^2}\right)$ rounds.

Next, we have to go over all $O\left(\frac{\log n}{\phi}\right)$ choices of $x$ and all $ O\left(\frac{\log^2 n}{\phi^2}\right)$ choices of $t$ to see if there is a pair $(t,j)$ meeting the required four conditions. More specifically, given $t$ and $x$, our task is the following.

\paragraph{Search for $j$ and $S_j(q_t)$.}
We need to compute the index $j$ that is the smallest index satisfying $\vol(S_j(q_t)) \geq (1+\phi)^x$, and then compute the set $S_j(q_t)$. We show that this can be done in  $O(\tlast \log n) =  O\left(\frac{\log^3 n}{\phi^2}\right)$ rounds via a ``random binary search'' on the vertex set  $U$ containing all vertices $u$ with $q_t(u) > 0$. 
For the sake of presentation, we rank all vertices $u_1, \ldots, u_{|U|}$ by decreasing order of $q_t(u) / \deg(u)$. Note that each $u_i$ does not know its rank $i$, and we cannot afford to compute the rank of all vertices in $U$. Also note that $S_i(q_t) = \{u_1, \ldots, u_i\}$.


We maintain two indices $L$ and $R$ that control the search space. Initially, $L \gets 1$ and $R \gets |U|$. In each iteration, we  pick one vertex $u_i$ from $\{u_L, \ldots, u_R\}$ uniformly at random, and calculate $\vol(S_i(q_t))$. This can be done in $O(\tlast)$ rounds. More specifically, we build a spanning tree $T$ of the edge set $P^\ast$ rooted at $v$, and use the tree for communication. It is clear that the subgraph induced by $P^\ast$ is connected and has diameter $O(\tlast)$.


If $\vol(S_i(q_t)) < (1+\phi)^x$, we update $L \gets i$; if $\vol(S_i(q_t)) = (1+\phi)^x$, we update $L \gets i$ and $R \gets i$; otherwise we update  $R \gets i-1$.  We are done when $L = R$.

In each iteration, with probability $1/2$ we sample $j$ in the middle half of $[L,R]$ and the size of search space 
$[L,R]$ shrinks by a factor of at least $3/4$. Therefore, w.h.p., 
after $O(\log n)$ iterations, we will have isolated $L = R = j$. Thus, the round complexity of this task is $O(\tlast \log n) =  O\left(\frac{\log^3 n}{\phi^2}\right)$.

\paragraph{Checking  (C.1*), (C.2*), and (C.3).} Given the index $j$ and the subset $S_j(q_t)$, it is straightforward to check these three conditions in $O(\tlast)$ rounds.

\paragraph{Checking  (C.4).}
We first note that this condition does not depend on $j$, and so we only need to do this test once for each $t$. Testing this condition can also be done via a random binary search, as described above, and this takes also $O(\tlast \log n) =  O\left(\frac{\log^3 n}{\phi^2}\right)$ rounds.


\paragraph{Round Complexity.} To summarize,  we go over all $O\left(\frac{\log n}{\phi}\right)$ choices of $x$ and all $ O\left(\frac{\log^2 n}{\phi^2}\right)$ choices of $t$, and for each pair $(t,x)$ we have to spend $O\left(\frac{\log^3 n}{\phi^2}\right)$ rounds. Therefore, the total round complexity is $O\left(\frac{\log^6 n}{\phi^5}\right)$.
\end{proof}

\begin{lemma}[Implementation of \balancedcut]\label{XXX-lem-parallel-nibble-impl}
The algorithm \parallelnibble$(G, \phi)$ can be implemented to run in $O\left(D \log n + \frac{\log^7 n}{\phi^5}\right)$ rounds in $\CONGEST$.
\end{lemma}
\begin{proof}
The implementation of \parallelnibble($G, \phi$) has three parts. 

\paragraph{Generation of \distnibble\ Instances.}
The first part is to generate all $k$ instances of \distnibble($G,v,\phi,b$), where the starting vertex $v \sim \psi_V$ is sampled according to the degree distribution, and $b \in [1, \ell]$ is sampled with $\Prob[b = i] = 2^{-i} / (1 - 2^{-\ell})$.

Following the idea of~\cite[Lemma 3.6]{ChangPZ19}, this task can be solved in $O(D + \log n)$ rounds, as follows. 
We build a BFS tree rooted at an arbitrary vertex $x$. For each vertex $v$, define $s(v)$ as the sum of $\deg(u)$ for each $u$ in the subtree rooted at $v$. In $O(D)$ rounds we can let each vertex $v$ learn the number $s(v)$ by a bottom-up traversal of the BFS tree. 

We let the root vertex $x$ sample the parameter $b$ for all $k$ instances of \distnibble.
Denote $K_i$ as the number of instances with $b = i$.
At the beginning, the root $x$ stores $K_i$ amount of $i$-tokens.
Let $L=\Theta(D)$ be the number of layers in the BFS tree. For $j = 1, \ldots, L$, the vertices of layer $j$ do the following. When an $i$-token arrives at $v$, 
the token disappears at $v$ with probability $\deg(v)/s(v)$
and $v$ locally generates an instance of \distnibble\ with starting vertex $v$ and parameter $b = i$;
otherwise, $v$ sends the token to a child $u$ 
with probability $\frac{s(u)}{s(v)-\deg(v)}$. 
Note that $v$ only needs to tell each child $u$ 
how many $i$-tokens $u$ gets.  Thus, for each $i$, the generation of all $K_i$ instances of \distnibble\ with a random starting vertex can be done in 
$L$ rounds. By pipelining, we can do this for all $i$ in $O(D+\log n)$ rounds, independent of $k$.

\paragraph{Simultaneous Execution of \distnibble.} The second part is to run all $k$ instances of \distnibble\ simultaneously. If there is an edge $e$ participating in more than $w = O(\log n)$ of them, then the two endpoints of $e$ broadcast a special message $\star$ to everyone else to notify them to terminate the algorithm with $C = \emptyset$, and the broadcasting takes $D$ rounds. Otherwise, this task can be done in $O(\log n) \cdot O\left(\frac{\log^6 n}{\phi^5}\right) = O\left(\frac{\log^7 n}{\phi^5}\right)$ rounds in view of Lemma~\ref{XXX-lem-dist-nibble-impl}. Overall, the round complexity is $O\left(D + \frac{\log^7 n}{\phi^5}\right)$.


\paragraph{Selection of $i^\ast$ and $C = U_{i^\ast}$.} In the description of the algorithm \parallelnibble($G, \phi$), we assume that all \distnibble\ instances are indexed from $1$ to $k$. However, in a distributed implementation we cannot afford to do this. What we can do is to let the starting vertex $v$ of each \distnibble\ instance locally generate a random $O(\log n)$-bit identifier associated with the \distnibble\ instance. We say that an \distnibble\ instance is the $i$th instance if its identifier is ranked $i$th in the increasing order of all $k$ identifiers. 
With these identifiers, we can now use a random binary search to find $i^\ast$ and calculate $C = U_{i^\ast}$ in $O(D \log n)$ rounds w.h.p.

\paragraph{Round Complexity.} To summarize, the round complexity for the three parts are $O(D+\log n)$, $O\left(D + \frac{\log^7 n}{\phi^5}\right)$, and $O(D \log n)$. Thus, the total round complexity is $O\left(D \log n + \frac{\log^7 n}{\phi^5}\right)$.
\end{proof}



\begin{lemma}[Implementation of \balancedcut]\label{XXX-lem-partition-nibble-impl}
The algorithm \balancedcut$(G, \phi, p)$ with $p = 1/\poly(n)$ can be implemented to run in $O\left(\frac{D \log^9 n}{\phi^4}+ \frac{\log^{15} n}{\phi^{9}}\right)$ rounds in $\CONGEST$.
\end{lemma}
\begin{proof}
This lemma follows immediately from Lemma~\ref{XXX-lem-parallel-nibble-impl}, as \balancedcut($G, \phi$) consists of 
\[s = O\left(g(\phi, \vol(V)) \log(1/p)\right)  = O\left(\frac{\log^8 n}{\phi^4}\right)\] iterations of \parallelnibble, where each of them costs $O\left(D \log n + \frac{\log^7 n}{\phi^5}\right)$ rounds, and so the total round complexity is  $O\left(\frac{D \log^9 n}{\phi^4}+ \frac{\log^{15} n}{\phi^{9}}\right)$.
\end{proof}

